Data-Efficient Pipeline for Offline Reinforcement Learning with Limited Data

Offline reinforcement learning (RL) can be used to improve future performance by leveraging historical data. There exist many different algorithms for offline RL, and it is well recognized that these algorithms, and their hyperparameter settings, can lead to decision policies with substantially differing performance. This prompts the need for pipelines that allow practitioners to systematically perform algorithm-hyperparameter selection for their setting. Critically, in most real-world settings, this pipeline must only involve the use of historical data. Inspired by statistical model selection methods for supervised learning, we introduce a task- and method-agnostic pipeline for automatically training, comparing, selecting, and deploying the best policy when the provided dataset is limited in size. In particular, our work highlights the importance of performing multiple data splits to produce more reliable algorithm-hyperparameter selection. While this is a common approach in supervised learning, to our knowledge, this has not been discussed in detail in the offline RL setting. We show it can have substantial impacts when the dataset is small. Compared to alternate approaches, our proposed pipeline outputs higher-performing deployed policies from a broad range of offline policy learning algorithms and across various simulation domains in healthcare, education, and robotics. This work contributes toward the development of a general-purpose meta-algorithm for automatic algorithm-hyperparameter selection for offline RL.

==> background.tex <==
\section{Background}
% Add notations and MDP definition. 
% \todo{Allen: write general section; Deon: add/change/edit notations to conform to MOPO}

We define a standard Markov Decision Process $M =$ $\langle \gS, A, T, r, \gamma \rangle$, where $\gS$ is a set of states; $A$ is a set of actions; $T: \gS \times A \rightarrow S$ is the transition dynamics; $r: \gS \times A \rightarrow \R$ is the reward function; $\gamma \in (0, 1)$ is the discount factor for future reward. Let $\tau = \{s_i, a_i, s_i', r_i\}_{i=0}^L$ be the trajectory sampled from $\pi$ on $M$, we want to learn a policy $\pi: \gS \rightarrow A$ that maximizes the expected return $V(\pi) = \E_{\tau \sim \rho_\pi}[\sum_{t=0}^\infty \gamma^t r(s_t, a_t)]$, where $\rho_\pi$ is the distribution of $\tau$ under policy $\pi$.

In an offline RL problem, we take a dataset: $\data = \{\tau_i\}_{i=1}^n$, which can be collected by one or a group of policies which we refer to as the behavior policy $\pi_b$ on the MDP $M$. The goal is to learn another policy $\pi_e$ from $\data$ that can perform better than $\pi_b$ when we deploy this policy in MDP $M$. $\pi_e$ is not allowed to interact with $M$ during policy learning.
We denote an offline policy learning algorithm and its associated learning settings, such as hyperparameters, model architecture, as $\mathcal{A}$. Borrowing notations from statistical learning, we can define $\mathcal{A}: \cup_{n=1}^\infty \{\tau\}^n \rightarrow (S \rightarrow A)$.
Algorithm $\mathcal{A}$ takes in $n$ trajectories and returns a policy: $\pi_e = \mathcal{A}(\data)$.
% Because we do not have access to the true MDP $M$, we apply different OPE algorithms $\hat V(\pi_e)$ to estimate this value.

% Emma can write this part a bit more??
One major difficulty in evaluating an offline reinforcement learning algorithm happens because the evaluation policy $\pi_e$ incurs a different state-action visitation distribution compared to the behavior policy $\pi_b$~\cite{fujimoto2019off}. We need to use a mismatched dataset to estimate the performance of $\pi_e$. This is called the Off-policy policy evaluation (OPE) problem. There are quite a few methods developed over the years. In our work, we focus on the class of importance-sampling based estimators, which we denote as $\hat V(\pi_e; \data)$. We refer readers to \citet{voloshin2019empirical} for a more comprehensive overview of these methods.
OPE estimates are sensitive to the properties of the dataset $\data$ and can introduce additional bias to our evaluation.
% I'm not very confident 

\subsection{Related works}

% Need to get Emma to read these...
% \paragraph{Off-policy Policy Evaluation} 

\paragraph{Offline Policy Learning}

\paragraph{Statistical Learning}

==> experiment.tex <==
\section{Environments}
\subsection{Sepsis}

\subsection{SmartTutor-Sim}

\subsection{SmartTutor}
To William: this is the smart primer stuff

\section{Experiments}


\begin{table*}[]
\centering
\begin{tabular}{@{}lcccccccc@{}}
\toprule
     & \multicolumn{4}{c}{N=200}                              & \multicolumn{4}{c}{N=1000}                                           \\ \midrule
             & $\delta$ & $P(A > A')$ & Intra Rank & Inter Rank       & $\delta$ & $P(A > A')$ & Intra Rank & \multicolumn{1}{l}{Inter Rank} \\ \midrule
2-fold CV    & 23.76    & 67.68\%     & 66.10\%    & 83.3\%           & 10.33    & 67.03\%     & 73.88\%    & 92.57\%                        \\
5-fold CV    & 15.61    & 65.36\%     & 61.11\%    & 75.0\%           & 6.58     & 68.83\%     & 69.14\%    & 76.30\%                        \\
10-fold CV   & 17.89    & 60.10\%     & 59.88\%    & 65.19\%          & 6.00     & 68.95\%     & 75.31\%    & 84.44\%                        \\ \midrule
Single Split & 31.48    & 66.02\%     & 68.53\%    & 65.64\%          & 12.41    & 63.40\%     & 63.84\%    & 68.00\%                        \\
2-split RS   & 28.81    & 67.74\%     & 68.93\%    & 73.0\%           & 9.10     & 66.00\%     & 71.10\%    & 78.65\%                        \\
5-split RS   & 28.76    & 70.38\%     & 69.10\%    & 81.65\%          & 8.47     & 67.23\%     & 71.90\%    & 95.91\%                        \\
10-split RS  & 28.20    & 71.30\%     & 71.60\%    & \textbf{92.40\%} & 7.90     & 68.92\%     & 78.24\%    & \textbf{99.26\%}               \\ \midrule
2x2 CV       & 22.73    & 69.45\%     & 65.28\%    & 77.61\%          & 9.66     & 68.20\%     & 72.01\%    & 93.08\%                        \\
5x2 CV       & 22.61    & 69.87\%     & 65.03\%    & 72.46\%          & 9.01     & 69.78\%     & 75.35\%    & 94.07\%                        \\
10x2 CV      & 22.11    & 70.10\%     & 70.22\%    & 68.70\%          & 8.66     & 70.05\%     & 79.26\%    & 97.96\%                        \\ \midrule
BCa (mean)   & 24.68    & 59.21\%     & 57.10\%    & 76.03\%          & 9.46     & 69.16\%     & 60.03\%    & 75.83\%                        \\
BCa (upper)  & ---      & 56.49\%     & 51.54\%    & 64.71\%          & ---      & 67.41\%     & 62.04\%    & 31.12\%                        \\
BCa (lower)  & ---      & 55.91\%     & 44.75\%    & 76.03\%          & ---      & 63.87\%     & 56.33\%    & 83.69\%                        \\ \bottomrule
\end{tabular}
\end{table*}

\begin{table*}[]
\centering
\begin{tabular}{@{}lcccc@{}}
\toprule
             & \multicolumn{4}{c}{Sepsis-MDP}                   \\ 
             & $\delta$ & $P(A > A')$ & Intra Rank & Inter Rank \\ \midrule
2-fold CV    & 33.44    &             &            &            \\
5-fold CV    & 17.44    & 73.29\%     & 78.19\%    & 67.41\%    \\ \midrule
Single Split & 31.14    & 24.27\%     & 42.72\%    & 84.92\%    \\
2-split RS   & 28.85    & 35.21\%     & 45.76\%    & 85.24\%    \\
5-split RS   & 23.17    & 51.62\%     & 61.44\%    & 86.98\%    \\
10-split RS  & 22.97    & 76.42\%     & 72.43\%    & 99.21\%    \\ \midrule
2x2 CV       & 24.06    &             &            &            \\
5x2 CV       & 19.80    &             &            &            \\
10x2 CV      & 18.73    &             &            &            \\ \bottomrule
\end{tabular}
\end{table*}

\begin{table*}[]
\centering
\begin{tabular}{@{}lcccc@{}}
\toprule
             & \multicolumn{4}{c}{Sepsis-POMDP}                 \\ \midrule
             & $\delta$ & $P(A > A')$ & Intra Rank & Inter Rank \\
10-fold CV   & 7.30     & 74.03\%     & 68.72\%    & 49.74\%    \\ \midrule
Single Split & 8.96     & 72.19\%     & 60.51\%    & 53.25\%    \\
2-split RS   & 7.72     & 73.19\%     & 62.70\%    & 52.75\%    \\
5-split RS   & 6.56     & 73.09\%     & 57.10\%    & 54.05\%    \\
10-split RS  & 5.76     & 72.64\%     & 57.20\%    & 51.32\%   \\ \bottomrule
\end{tabular}
\caption{Sepsis-POMDP N=5000, WIS.}
\end{table*}

\begin{table*}[]
\centering
\begin{tabular}{l|cc|cc|cc|cc}
\toprule
\multicolumn{1}{c}{} & \multicolumn{6}{c}{Sepsis-POMDP}                                                                      & \multicolumn{2}{c}{Sepsis-MDP} \\
\multicolumn{1}{c}{} & \multicolumn{2}{c}{N=200}                   & \multicolumn{2}{c}{N=1000} & \multicolumn{2}{c}{N=5000} & \multicolumn{2}{c}{N=200}      \\ \midrule
\multicolumn{1}{c}{} & \multicolumn{1}{r}{Estimated} & True & Estimated   & True  & Estimated   & True  & Estimated     & True     \\ \midrule
Single Split         & 53.2                          & -26.4       & 84.62       & -32.0        & 91.22       & -61.6        & 63.92         & -20.12         \\
10-split RS          & 24.89                         & -7.8        & 11.92       & 6.96         & 10.77       & -5.52        & ---           & -2.14          \\
10-fold CV           & 24.76                         & -19.2       & 10.95       & 5.32         & 11.42       & -7.00        &               &                \\ \bottomrule
\end{tabular}
\end{table*}

% 1-split,22.1,52.4,14.3,4.8
\begin{table*}[]
\centering
\begin{tabular}{@{}ccccc@{}}
\toprule
\multicolumn{1}{l}{Procedure} & $\delta$ & $P(A > A')$ & Intra-Rank & Inter-Rank \\ \midrule
Single split      & 22.1     & 52.4        & 14.3       & 4.8       \\ \midrule
2-fold                        & 21.5     & 68.3        & 52.4       & 14.3       \\
5-fold                        & 15.3     & 61.9        & 14.3       & 4.8        \\ \midrule
2-split                       & 16.2     & 66.2        & 57.6       & 27.4       \\
5-split                       & 14.5     & 68.4        & 47.9       & 23.1       \\
10-split                      & 12.7     & 68.3        & 33.3       & 33.3       \\ \bottomrule
\end{tabular}
\caption{Robomimic dataset, PH, Transport, N=200. Single-split we report worst split performance.}
\end{table*}

\begin{table*}[]
\centering
\begin{tabular}{@{}ccccc@{}}
\multicolumn{1}{l}{} & \multicolumn{4}{c}{Robomimic - Transport}   \\ \midrule
Procedure            & Algorithm  & Estimated & Half (Avg) & Full  \\ \midrule
2-fold               & CQL-Exp4   & 1.226       & 0.0        & 0.0   \\
5-fold               & CQL-Exp6   & 0.144       & 0.0        & 0.0   \\ \midrule
1-split              & CQL-Exp3   & 0.514     & 0.0      & 0.0 \\ 
2-split              & CQL-Exp2   & 0.111     & 0.0      & 0.0 \\
5-split              & CQL-Exp6   & 0.198     & 0.0      & 0.0 \\
10-split             & BCRNN-Exp3 & 0.112     & 0.0      & 0.0 \\ \bottomrule
\end{tabular}
\caption{Robomimic dataset, PH, Transport, N=200.}
\end{table*}

\begin{table*}[]
\centering
\begin{tabular}{@{}ccccc@{}}
\toprule
Procedure & $\delta$ & $P(A > A')$ & Intra-Rank & Inter-Rank \\ \midrule
5-fold    & 11.0     & 38.1        & 43.2       & 51.9       \\
10-fold   & 11.9     & 63.6        & 60.5       & 92.6       \\ \midrule
1-split   & 17.5     & 60.4        & 56.1       & 87.0       \\
2-split   & 12.5     & 60.6        & 61.8       & 89.1       \\
5-split   & 12.8     & 67.5        & 68.4       & 94.9       \\
10-split  & 12.5     & 68.9        & 74.1       & 91.4       \\ \bottomrule
\end{tabular}
\caption{TutorBot, N=200, Uniform Policy. Weighted Importance Sampling. Single split we report average.}
\end{table*}

\begin{table*}[]
\centering
\begin{tabular}{@{}lllll@{}}
\toprule
Procedure & Algorithm      & Estimated & Half (Avg) & Full  \\ \midrule
5-fold    & pg-exp-0       & 1.331     & 1.243      & 1.188 \\
10-fold   & bcminipg-exp-4 & 1.703     & 1.304      & 1.389 \\ \midrule
1-split   & bcminipg-exp-3 & 1.471     & 1.239      & 1.337 \\
2-split   & bcminipg-exp-8 & 2.305     & 1.149      & 1.434 \\
5-split   & bcminipg-exp-8 & 1.463     & 1.251      & 1.434 \\
10-split  & bcminipg-exp-3 & 1.451     & 1.192      & 1.337 \\ \bottomrule
\end{tabular}
\caption{TutorBot, N=200, Uniform Policy. Weighted Importance Sampling. Single split we report average.}
\end{table*}

\begin{table*}[]
\centering
\begin{tabular}{@{}ccccc@{}}
\toprule
Procedure & Algorithm      & Estimated & Half (Avg) & Full  \\ \midrule
5-fold    & pg-exp-0       & 1.331     & 1.243      & 1.188 \\
10-fold   & bcminipg-exp-4 & 1.703     & 1.304      & 1.389 \\ \midrule 
1-split   & bcminipg-exp-3 & 1.471     & 1.239      & 1.337 \\
2-split   & bcminipg-exp-3 & 1.564     & 1.178      & 1.337 \\
5-split   & bcminipg-exp-3 & 1.657     & 1.180      & 1.337 \\
10-split  & bcminipg-exp-3 & 1.451     & 1.192      & 1.337 \\ \bottomrule
\end{tabular}
\caption{TutorBot, N=200, Uniform Policy. Weighted Importance Sampling. Single split we report average.}
\end{table*}

\begin{table*}[]
\centering
\begin{tabular}{@{}ccccc@{}}
\toprule
Procedure & $\delta$ & $P(A > A')$ & Intra-Rank & Inter-Rank \\ \midrule
2-fold    & 42.2     & 82.5        & 71.4       & 100.0      \\
5-fold    & 39.5     & 93.7        & 85.7       & 100.0      \\ \midrule
1-split   & 55.0     & 74.5        & 66.9       & 78.1       \\
2-split   & 53.1     & 79.6        & 79.0       & 92.4       \\
5-split   & 50.7     & 81.3        & 83.8       & 95.5       \\
10-split  & 50.7     & 81.0        & 90.5       & 95.2       \\ \bottomrule
\end{tabular}
\caption{Robomimic dataset, PH, Can-Paired, N=200.}
\end{table*}

\begin{table*}[]
\centering
\begin{tabular}{@{}ccccc@{}}
\toprule
Procedure & Algorithm   & Estimated & Half (Avg) & Full  \\ \midrule
2-fold    & bcrnn-exp-3 & 2.158     & 0.450      & 0.700 \\
5-fold    & bcrnn-exp-3 & 1.897     & 0.520      & 0.700 \\ \midrule
1-split   & bcrnn-exp-1 & 2.008     & 0.400      & 0.500 \\
2-split   & bcrnn-exp-2 & 2.528     & 0.500      & 0.700 \\
5-split   & bcrnn-exp-3 & 2.161     & 0.420      & 0.700 \\
10-split  & bcrnn-exp-3 & 2.125     & 0.390      & 0.700 \\ \bottomrule
\end{tabular}
\caption{Robomimic dataset, PH, Can-Paired, N=200.}
\end{table*}

\begin{table*}[]
\centering
\begin{tabular}{@{}ccccc@{}}
\toprule
Procedure & Algorithm    & Estimated & Half (Avg) & Full  \\ \midrule
5-fold    & mbsqi-exp-17 & 26.0      & -18.0      & -16.1 \\
10-fold   & bcq-exp-5    & 49.5      & -16.3      & -21.2 \\
1-split   & mdp-exp-6    & 68.1      & -41.8      & -36.2 \\
2-split   & mdp-exp-0    & 36.5      & -37.2      & -35.1 \\
5-split   & mbsqi-exp-59 & 24.4      & -17.8      & -15.2 \\
10-split  & bcq-exp-25   & 24.9      & -10.2      & -9.1  \\ \bottomrule
\end{tabular}
\caption{Sepsis-POMDP N=200, WIS.}
\end{table*}

\begin{table*}[]
\centering
\begin{tabular}{@{}ccccc@{}}
\toprule
Procedure & Algorithm    & Estimated & Half (Avg) & Full  \\ \midrule
5-fold    & bcq-exp-1    & 16.8      & 0.4        & -1.9  \\
10-fold   & mdp-exp-18   & 21.7      & -0.2       & 0.6   \\ \midrule
1-split   & mbsqi-exp-29 & 35.1      & -37.8      & -21.8 \\
2-split   & mbsqi-exp-80 & 18.0      & 5.1        & 5.5   \\
5-split   & mbsqi-exp-80 & 14.7      & 5.1        & 5.5   \\
10-split  & mbsqi-exp-78 & 11.9      & 4.8        & 7.2   \\ \bottomrule
\end{tabular}
\caption{Sepsis-POMDP N=1000, WIS.}
\end{table*}

\begin{table*}[]
\centering
\begin{tabular}{@{}ccccc@{}}
\toprule
Procedure & Algorithm & Estimated & Half (Avg) & Full \\ \midrule
5-fold    & mdp-exp-0 & 54.8      & 5.5        & 5.7  \\
10-fold   & mdp-exp-2 & 52.7      & 7.2        & 9.1  \\ \midrule
1-split   & mdp-exp-0 & 78.0      & 10.9       & 5.7  \\
2-split   & mdp-exp-6 & 47.4      & 12.1       & 12.7 \\
5-split   & mdp-exp-6 & 49.6      & 9.1        & 12.7 \\
10-split  & mdp-exp-6 & 44.2      & 12.3       & 12.7 \\ \bottomrule
\end{tabular}
\caption{Sepsis-POMDP N=5000, WIS.}
\end{table*}

\begin{table*}[]
\centering
\begin{tabular}{@{}lllll@{}}
\toprule
Procedure & Algorithm   & Estimated & Half (Avg) & Full  \\ \midrule
2-fold    & bcrnn-exp-3 & 2.158     & 0.450      & 0.711 \\
5-fold    & bcrnn-exp-3 & 1.897     & 0.520      & 0.711 \\ \midrule
1-split   & bcrnn-exp-2 & 2.444     & 0.200      & 0.700 \\ 
2-split   & iris-exp-0  & 2.641     & 0.600      & 0.722 \\
5-split   & iris-exp-0  & 2.170     & 0.540      & 0.722 \\
10-split  & iris-exp-0  & 2.126     & 0.540      & 0.722 \\ \bottomrule
\end{tabular}
\caption{Robomimic Can-Paired, FQE}
\end{table*}



==> fvcxkgstnhxcyccfvtcknzrmdvqdfdgy_arXiv/algorithm.tex <==







\noindent\makebox[\textwidth][c]{
\begin{minipage}{0.55\textwidth}
\centering
\begin{algorithm}[H]
\SetAlgoLined
\SetKwFunction{subsample}{Subsample}
\SetKwFunction{append}{append}
\KwIn{offline RL data $\data$; set of AH pairs [$\gA_1, \gA_2, ..., \gA_z$], OPE estimator  $\widehat V$, split number $K\in \mathbb{N}$.}
\KwOut{policy $\hat \pi^*$ for deployment}
\BlankLine
$\gR$ = $\emptyset$\\ %
\For{$i \leftarrow 1...K$}{
    $R^\mathrm{train}_i, R^\mathrm{valid}_i = $ \subsample($\data, 0.5$) \\
    $\gR = \gR \cup (R^\mathrm{train}_i, R^\mathrm{valid}_i)$
}
$\gG$ = []  \\ %
\For{$i \leftarrow 1...z$}{
    $\gS$ = [] \\
    \For{$j \leftarrow 1...K$}{
        $\pi_i = \mathcal{A}(R^\mathrm{train}_j)$ \\
        $\gS_{ij} = \widehat V(\pi_i; R^\mathrm{valid}_j)$ \\
     }
     $\gG_i = \frac{1}{K} \sum_{j=1}^K \gS_{ij}$
 }
  $\gA^* = \gA_{o+}$ where $o = \argmax(\gG)$\\
 $\pi^* = \gA^*(\data)$  \\ %
 \Return{$\pi^*$}
 \caption{\ssrrrs: $\gA_i$ Selection with Repeated Random Sub-sampling}
 \label{alg:ssr-rs}
\end{algorithm}

\end{minipage}
}

==> fvcxkgstnhxcyccfvtcknzrmdvqdfdgy_arXiv/background.tex <==
\section{Background}

We define a standard Markov Decision Process $M =$ $\langle \gS, A, T, r, \gamma \rangle$, where $\gS$ is a set of states; $A$ is a set of actions; $T: \gS \times A \rightarrow S$ is the transition dynamics; $r: \gS \times A \rightarrow \R$ is the reward function; $\gamma \in (0, 1)$ is the discount factor for future reward. Let $\tau = \{s_i, a_i, s_i', r_i\}_{i=0}^L$ be the trajectory sampled from $\pi$ on $M$, we want to learn a policy $\pi: \gS \rightarrow A$ that maximizes the expected return $V(\pi) = \E_{\tau \sim \rho_\pi}[\sum_{t=0}^\infty \gamma^t r(s_t, a_t)]$, where $\rho_\pi$ is the distribution of $\tau$ under policy $\pi$.

In an offline RL problem, we take a dataset: $\data = \{\tau_i\}_{i=1}^n$, which can be collected by one or a group of policies which we refer to as the behavior policy $\pi_b$ on the MDP $M$. The goal is to learn another policy $\pi_e$ from $\data$ that can perform better than $\pi_b$ when we deploy this policy in MDP $M$. $\pi_e$ is not allowed to interact with $M$ during policy learning.
We denote an offline policy learning algorithm and its associated learning settings, such as hyperparameters, model architecture, as $\mathcal{A}$. Borrowing notations from statistical learning, we can define $\mathcal{A}: \cup_{n=1}^\infty \{\tau\}^n \rightarrow (S \rightarrow A)$.
Algorithm $\mathcal{A}$ takes in $n$ trajectories and returns a policy: $\pi_e = \mathcal{A}(\data)$.

One major difficulty in evaluating an offline reinforcement learning algorithm happens because the evaluation policy $\pi_e$ incurs a different state-action visitation distribution compared to the behavior policy $\pi_b$~\cite{fujimoto2019off}. We need to use a mismatched dataset to estimate the performance of $\pi_e$. This is called the Off-policy policy evaluation (OPE) problem. There are quite a few methods developed over the years. In our work, we focus on the class of importance-sampling based estimators, which we denote as $\hat V(\pi_e; \data)$. We refer readers to \citet{voloshin2019empirical} for a more comprehensive overview of these methods.
OPE estimates are sensitive to the properties of the dataset $\data$ and can introduce additional bias to our evaluation.

\subsection{Related works}


\paragraph{Offline Policy Learning}

\paragraph{Statistical Learning}

==> fvcxkgstnhxcyccfvtcknzrmdvqdfdgy_arXiv/checklist.tex <==
\section*{Checklist}




\begin{enumerate}


\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{See Section~\ref{sec:results} and Section~\ref{sec:discussion}.}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerNA{}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}


\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerYes{See Section~\ref{sec:theory} and Section~\ref{ap:proof}.}
        \item Did you include complete proofs of all theoretical results?
    \answerYes{See Section~\ref{sec:theory} and Section~\ref{ap:proof}.}
\end{enumerate}


\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)? \answerYes{See Supplementary Material.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{See Sections~\ref{sec:exp},~\ref{ap:domains},~\ref{ap:exp2},~\ref{ap:exp3},~\ref{ap:exp4} and~\ref{ap:exp5}}
    \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{}
    \item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{}
\end{enumerate}


\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{}
  \item Did you mention the license of the assets?
    \answerNA{Open-source}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYes{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}


\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}


\end{enumerate}


==> fvcxkgstnhxcyccfvtcknzrmdvqdfdgy_arXiv/discussion.tex <==
\section{Discussion and Conclusion}
\label{sec:discussion}




We presented \ssr, a pipeline for training, comparing, selecting and deploying offline RL policies in a small data regime. The approach performs automated \ah selection with a robust hyperparameter evaluation process using repeated random sub-sampling. \ssr allows to consistently and reliably deploy best-performing policies thanks to jointly avoiding overfitting on a single dataset split and being data efficient in re-using the whole dataset for final training. We prove that a single split has a high failure rate of discovering the optimal \ah because of reward sparsity. We have demonstrated its strong empirical performance across multiple and various challenging domains, including real-world applications where \ah tuning cannot be performed online.

There exist many interesting areas for future work. The proposed offline RL pipeline assumes the user/practitioner has selected a particular OPE method. OPE is an important subarea of its own and different approaches have different bias/variance tradeoffs. Recent work on automated model selection algorithms for OPE~\citep{su2020adaptive,lee2021model} are a promising approach for producing good internal estimators. A second issue is that while our approach aims to produce a high-performing policy, it does not also produce an accurate estimate of this policy since the entire dataset is used at the end for training. An interesting issue is whether cross-splitting~\citep{chernozhukov2016double} or other methods could be used to compute reliable estimators as well as perform policy optimization. %






==> fvcxkgstnhxcyccfvtcknzrmdvqdfdgy_arXiv/experiment.tex <==
\section{Environments}
\subsection{Sepsis}

\subsection{SmartTutor-Sim}

\subsection{SmartTutor}
To William: this is the smart primer stuff

\section{Experiments}


\begin{table*}[]
\centering
\begin{tabular}{@{}lcccccccc@{}}
\toprule
     & \multicolumn{4}{c}{N=200}                              & \multicolumn{4}{c}{N=1000}                                           \\ \midrule
             & $\delta$ & $P(A > A')$ & Intra Rank & Inter Rank       & $\delta$ & $P(A > A')$ & Intra Rank & \multicolumn{1}{l}{Inter Rank} \\ \midrule
2-fold CV    & 23.76    & 67.68\%     & 66.10\%    & 83.3\%           & 10.33    & 67.03\%     & 73.88\%    & 92.57\%                        \\
5-fold CV    & 15.61    & 65.36\%     & 61.11\%    & 75.0\%           & 6.58     & 68.83\%     & 69.14\%    & 76.30\%                        \\
10-fold CV   & 17.89    & 60.10\%     & 59.88\%    & 65.19\%          & 6.00     & 68.95\%     & 75.31\%    & 84.44\%                        \\ \midrule
Single Split & 31.48    & 66.02\%     & 68.53\%    & 65.64\%          & 12.41    & 63.40\%     & 63.84\%    & 68.00\%                        \\
2-split RS   & 28.81    & 67.74\%     & 68.93\%    & 73.0\%           & 9.10     & 66.00\%     & 71.10\%    & 78.65\%                        \\
5-split RS   & 28.76    & 70.38\%     & 69.10\%    & 81.65\%          & 8.47     & 67.23\%     & 71.90\%    & 95.91\%                        \\
10-split RS  & 28.20    & 71.30\%     & 71.60\%    & \textbf{92.40\%} & 7.90     & 68.92\%     & 78.24\%    & \textbf{99.26\%}               \\ \midrule
2x2 CV       & 22.73    & 69.45\%     & 65.28\%    & 77.61\%          & 9.66     & 68.20\%     & 72.01\%    & 93.08\%                        \\
5x2 CV       & 22.61    & 69.87\%     & 65.03\%    & 72.46\%          & 9.01     & 69.78\%     & 75.35\%    & 94.07\%                        \\
10x2 CV      & 22.11    & 70.10\%     & 70.22\%    & 68.70\%          & 8.66     & 70.05\%     & 79.26\%    & 97.96\%                        \\ \midrule
BCa (mean)   & 24.68    & 59.21\%     & 57.10\%    & 76.03\%          & 9.46     & 69.16\%     & 60.03\%    & 75.83\%                        \\
BCa (upper)  & ---      & 56.49\%     & 51.54\%    & 64.71\%          & ---      & 67.41\%     & 62.04\%    & 31.12\%                        \\
BCa (lower)  & ---      & 55.91\%     & 44.75\%    & 76.03\%          & ---      & 63.87\%     & 56.33\%    & 83.69\%                        \\ \bottomrule
\end{tabular}
\end{table*}

\begin{table*}[]
\centering
\begin{tabular}{@{}lcccc@{}}
\toprule
             & \multicolumn{4}{c}{Sepsis-MDP}                   \\ 
             & $\delta$ & $P(A > A')$ & Intra Rank & Inter Rank \\ \midrule
2-fold CV    & 33.44    &             &            &            \\
5-fold CV    & 17.44    & 73.29\%     & 78.19\%    & 67.41\%    \\ \midrule
Single Split & 31.14    & 24.27\%     & 42.72\%    & 84.92\%    \\
2-split RS   & 28.85    & 35.21\%     & 45.76\%    & 85.24\%    \\
5-split RS   & 23.17    & 51.62\%     & 61.44\%    & 86.98\%    \\
10-split RS  & 22.97    & 76.42\%     & 72.43\%    & 99.21\%    \\ \midrule
2x2 CV       & 24.06    &             &            &            \\
5x2 CV       & 19.80    &             &            &            \\
10x2 CV      & 18.73    &             &            &            \\ \bottomrule
\end{tabular}
\end{table*}

\begin{table*}[]
\centering
\begin{tabular}{@{}lcccc@{}}
\toprule
             & \multicolumn{4}{c}{Sepsis-POMDP}                 \\ \midrule
             & $\delta$ & $P(A > A')$ & Intra Rank & Inter Rank \\
10-fold CV   & 7.30     & 74.03\%     & 68.72\%    & 49.74\%    \\ \midrule
Single Split & 8.96     & 72.19\%     & 60.51\%    & 53.25\%    \\
2-split RS   & 7.72     & 73.19\%     & 62.70\%    & 52.75\%    \\
5-split RS   & 6.56     & 73.09\%     & 57.10\%    & 54.05\%    \\
10-split RS  & 5.76     & 72.64\%     & 57.20\%    & 51.32\%   \\ \bottomrule
\end{tabular}
\caption{Sepsis-POMDP N=5000, WIS.}
\end{table*}

\begin{table*}[]
\centering
\begin{tabular}{l|cc|cc|cc|cc}
\toprule
\multicolumn{1}{c}{} & \multicolumn{6}{c}{Sepsis-POMDP}                                                                      & \multicolumn{2}{c}{Sepsis-MDP} \\
\multicolumn{1}{c}{} & \multicolumn{2}{c}{N=200}                   & \multicolumn{2}{c}{N=1000} & \multicolumn{2}{c}{N=5000} & \multicolumn{2}{c}{N=200}      \\ \midrule
\multicolumn{1}{c}{} & \multicolumn{1}{r}{Estimated} & True & Estimated   & True  & Estimated   & True  & Estimated     & True     \\ \midrule
Single Split         & 53.2                          & -26.4       & 84.62       & -32.0        & 91.22       & -61.6        & 63.92         & -20.12         \\
10-split RS          & 24.89                         & -7.8        & 11.92       & 6.96         & 10.77       & -5.52        & ---           & -2.14          \\
10-fold CV           & 24.76                         & -19.2       & 10.95       & 5.32         & 11.42       & -7.00        &               &                \\ \bottomrule
\end{tabular}
\end{table*}

\begin{table*}[]
\centering
\begin{tabular}{@{}ccccc@{}}
\toprule
\multicolumn{1}{l}{Procedure} & $\delta$ & $P(A > A')$ & Intra-Rank & Inter-Rank \\ \midrule
Single split      & 22.1     & 52.4        & 14.3       & 4.8       \\ \midrule
2-fold                        & 21.5     & 68.3        & 52.4       & 14.3       \\
5-fold                        & 15.3     & 61.9        & 14.3       & 4.8        \\ \midrule
2-split                       & 16.2     & 66.2        & 57.6       & 27.4       \\
5-split                       & 14.5     & 68.4        & 47.9       & 23.1       \\
10-split                      & 12.7     & 68.3        & 33.3       & 33.3       \\ \bottomrule
\end{tabular}
\caption{Robomimic dataset, PH, Transport, N=200. Single-split we report worst split performance.}
\end{table*}

\begin{table*}[]
\centering
\begin{tabular}{@{}ccccc@{}}
\multicolumn{1}{l}{} & \multicolumn{4}{c}{Robomimic - Transport}   \\ \midrule
Procedure            & Algorithm  & Estimated & Half (Avg) & Full  \\ \midrule
2-fold               & CQL-Exp4   & 1.226       & 0.0        & 0.0   \\
5-fold               & CQL-Exp6   & 0.144       & 0.0        & 0.0   \\ \midrule
1-split              & CQL-Exp3   & 0.514     & 0.0      & 0.0 \\ 
2-split              & CQL-Exp2   & 0.111     & 0.0      & 0.0 \\
5-split              & CQL-Exp6   & 0.198     & 0.0      & 0.0 \\
10-split             & BCRNN-Exp3 & 0.112     & 0.0      & 0.0 \\ \bottomrule
\end{tabular}
\caption{Robomimic dataset, PH, Transport, N=200.}
\end{table*}

\begin{table*}[]
\centering
\begin{tabular}{@{}ccccc@{}}
\toprule
Procedure & $\delta$ & $P(A > A')$ & Intra-Rank & Inter-Rank \\ \midrule
5-fold    & 11.0     & 38.1        & 43.2       & 51.9       \\
10-fold   & 11.9     & 63.6        & 60.5       & 92.6       \\ \midrule
1-split   & 17.5     & 60.4        & 56.1       & 87.0       \\
2-split   & 12.5     & 60.6        & 61.8       & 89.1       \\
5-split   & 12.8     & 67.5        & 68.4       & 94.9       \\
10-split  & 12.5     & 68.9        & 74.1       & 91.4       \\ \bottomrule
\end{tabular}
\caption{TutorBot, N=200, Uniform Policy. Weighted Importance Sampling. Single split we report average.}
\end{table*}

\begin{table*}[]
\centering
\begin{tabular}{@{}lllll@{}}
\toprule
Procedure & Algorithm      & Estimated & Half (Avg) & Full  \\ \midrule
5-fold    & pg-exp-0       & 1.331     & 1.243      & 1.188 \\
10-fold   & bcminipg-exp-4 & 1.703     & 1.304      & 1.389 \\ \midrule
1-split   & bcminipg-exp-3 & 1.471     & 1.239      & 1.337 \\
2-split   & bcminipg-exp-8 & 2.305     & 1.149      & 1.434 \\
5-split   & bcminipg-exp-8 & 1.463     & 1.251      & 1.434 \\
10-split  & bcminipg-exp-3 & 1.451     & 1.192      & 1.337 \\ \bottomrule
\end{tabular}
\caption{TutorBot, N=200, Uniform Policy. Weighted Importance Sampling. Single split we report average.}
\end{table*}

\begin{table*}[]
\centering
\begin{tabular}{@{}ccccc@{}}
\toprule
Procedure & Algorithm      & Estimated & Half (Avg) & Full  \\ \midrule
5-fold    & pg-exp-0       & 1.331     & 1.243      & 1.188 \\
10-fold   & bcminipg-exp-4 & 1.703     & 1.304      & 1.389 \\ \midrule 
1-split   & bcminipg-exp-3 & 1.471     & 1.239      & 1.337 \\
2-split   & bcminipg-exp-3 & 1.564     & 1.178      & 1.337 \\
5-split   & bcminipg-exp-3 & 1.657     & 1.180      & 1.337 \\
10-split  & bcminipg-exp-3 & 1.451     & 1.192      & 1.337 \\ \bottomrule
\end{tabular}
\caption{TutorBot, N=200, Uniform Policy. Weighted Importance Sampling. Single split we report average.}
\end{table*}

\begin{table*}[]
\centering
\begin{tabular}{@{}ccccc@{}}
\toprule
Procedure & $\delta$ & $P(A > A')$ & Intra-Rank & Inter-Rank \\ \midrule
2-fold    & 42.2     & 82.5        & 71.4       & 100.0      \\
5-fold    & 39.5     & 93.7        & 85.7       & 100.0      \\ \midrule
1-split   & 55.0     & 74.5        & 66.9       & 78.1       \\
2-split   & 53.1     & 79.6        & 79.0       & 92.4       \\
5-split   & 50.7     & 81.3        & 83.8       & 95.5       \\
10-split  & 50.7     & 81.0        & 90.5       & 95.2       \\ \bottomrule
\end{tabular}
\caption{Robomimic dataset, PH, Can-Paired, N=200.}
\end{table*}

\begin{table*}[]
\centering
\begin{tabular}{@{}ccccc@{}}
\toprule
Procedure & Algorithm   & Estimated & Half (Avg) & Full  \\ \midrule
2-fold    & bcrnn-exp-3 & 2.158     & 0.450      & 0.700 \\
5-fold    & bcrnn-exp-3 & 1.897     & 0.520      & 0.700 \\ \midrule
1-split   & bcrnn-exp-1 & 2.008     & 0.400      & 0.500 \\
2-split   & bcrnn-exp-2 & 2.528     & 0.500      & 0.700 \\
5-split   & bcrnn-exp-3 & 2.161     & 0.420      & 0.700 \\
10-split  & bcrnn-exp-3 & 2.125     & 0.390      & 0.700 \\ \bottomrule
\end{tabular}
\caption{Robomimic dataset, PH, Can-Paired, N=200.}
\end{table*}

\begin{table*}[]
\centering
\begin{tabular}{@{}ccccc@{}}
\toprule
Procedure & Algorithm    & Estimated & Half (Avg) & Full  \\ \midrule
5-fold    & mbsqi-exp-17 & 26.0      & -18.0      & -16.1 \\
10-fold   & bcq-exp-5    & 49.5      & -16.3      & -21.2 \\
1-split   & mdp-exp-6    & 68.1      & -41.8      & -36.2 \\
2-split   & mdp-exp-0    & 36.5      & -37.2      & -35.1 \\
5-split   & mbsqi-exp-59 & 24.4      & -17.8      & -15.2 \\
10-split  & bcq-exp-25   & 24.9      & -10.2      & -9.1  \\ \bottomrule
\end{tabular}
\caption{Sepsis-POMDP N=200, WIS.}
\end{table*}

\begin{table*}[]
\centering
\begin{tabular}{@{}ccccc@{}}
\toprule
Procedure & Algorithm    & Estimated & Half (Avg) & Full  \\ \midrule
5-fold    & bcq-exp-1    & 16.8      & 0.4        & -1.9  \\
10-fold   & mdp-exp-18   & 21.7      & -0.2       & 0.6   \\ \midrule
1-split   & mbsqi-exp-29 & 35.1      & -37.8      & -21.8 \\
2-split   & mbsqi-exp-80 & 18.0      & 5.1        & 5.5   \\
5-split   & mbsqi-exp-80 & 14.7      & 5.1        & 5.5   \\
10-split  & mbsqi-exp-78 & 11.9      & 4.8        & 7.2   \\ \bottomrule
\end{tabular}
\caption{Sepsis-POMDP N=1000, WIS.}
\end{table*}

\begin{table*}[]
\centering
\begin{tabular}{@{}ccccc@{}}
\toprule
Procedure & Algorithm & Estimated & Half (Avg) & Full \\ \midrule
5-fold    & mdp-exp-0 & 54.8      & 5.5        & 5.7  \\
10-fold   & mdp-exp-2 & 52.7      & 7.2        & 9.1  \\ \midrule
1-split   & mdp-exp-0 & 78.0      & 10.9       & 5.7  \\
2-split   & mdp-exp-6 & 47.4      & 12.1       & 12.7 \\
5-split   & mdp-exp-6 & 49.6      & 9.1        & 12.7 \\
10-split  & mdp-exp-6 & 44.2      & 12.3       & 12.7 \\ \bottomrule
\end{tabular}
\caption{Sepsis-POMDP N=5000, WIS.}
\end{table*}

\begin{table*}[]
\centering
\begin{tabular}{@{}lllll@{}}
\toprule
Procedure & Algorithm   & Estimated & Half (Avg) & Full  \\ \midrule
2-fold    & bcrnn-exp-3 & 2.158     & 0.450      & 0.711 \\
5-fold    & bcrnn-exp-3 & 1.897     & 0.520      & 0.711 \\ \midrule
1-split   & bcrnn-exp-2 & 2.444     & 0.200      & 0.700 \\ 
2-split   & iris-exp-0  & 2.641     & 0.600      & 0.722 \\
5-split   & iris-exp-0  & 2.170     & 0.540      & 0.722 \\
10-split  & iris-exp-0  & 2.126     & 0.540      & 0.722 \\ \bottomrule
\end{tabular}
\caption{Robomimic Can-Paired, FQE}
\end{table*}



==> fvcxkgstnhxcyccfvtcknzrmdvqdfdgy_arXiv/experiment_new.tex <==
\section{Experiments}
\label{sec:exp}
\looseness=-1 In this section, we answer the following questions: (a) how does the pipeline \ssrrrs compare to other methods? (b) does the proposed pipeline for $\mathcal{A}_i$ selection and policy deployment allow us to generate the best policy trained on the whole dataset? (c) does re-training on the whole dataset (data efficiency) generate better policies than policies trained on half of the dataset when $\mathcal{A}_i$ is selected by the pipeline? In addition, we conduct two ablation studies to answer to: what number of splits should we use for \ssrrrs, and what is the impact of dataset size on the pipeline results? 


\subsection{Task/Domains}
\looseness=-1 The experimental evaluation involves a variety of real-world and simulated domains, ranging from tabular settings to continuous control robotics environments. We evaluate the performance of \ssr in selecting the best algorithm regardless of task domains and assumptions on task structure. We conduct experiments on eight datasets (Figure~\ref{fig:ssr-tasks}) from five domains (details in Appendix~\ref{ap:domains}), which we give a short description below, and use as many as 540 candidate \ah pairs for the Sepsis POMDP domain.

\begin{figure*}[ht!]%
    \centering
    \includegraphics[width=0.9\linewidth]{images/ssr-tasks.pdf}
    \caption{Illustrations from left to right of the D4RL, Robomimic, TutorBot and Sepsis domains.}
    \label{fig:ssr-tasks}
\end{figure*}

\textbf{Sepsis.}
The first domain is based on the simulator and work by \cite{oberst2019counterfactual} and revolves around treating sepsis patients. The goal of the policy for this simulator is to discharge patients from the hospital.
In this domain, we experiment on two tasks: \underline{Sepsis-MDP} and \underline{Sepsis-POMDP}, a POMDP version of Sepsis-MDP.







\textbf{TutorBot.}
The second domain includes a \underline{TutorBot} simulator that is designed to support 3-5th grade elementary school children in understanding the concept of volume and engaging them while doing so. An online study was conducted using a policy-gradient-based RL agent, which interacted with about 200 students.
We took the observations from this online study and built a simulator that reflects student learning progression, combined with some domain knowledge.%

    

\looseness=-1\textbf{Robomimic.}
Robomimic~\citep{mandlekar2021what} is composed of various continuous control robotics environments with suboptimal human data. We use the \underline{Can-Paired} and \underline{Transport} dataset composed of 200 mixed-quality human demonstrations. 
~\citet{mandlekar2021what} attempted to use the RL objective loss on a 20\% split validation set to select the best \ah pair, but reported that the selected \ah did not perform well in the simulator, which makes this task an interesting testbed for our pipeline. 

\looseness=-1\textbf{D4RL.}
D4RL~\citep{fu2020d4rl} is an offline RL standardized benchmark designed and commonly used to evaluate the progress of offline RL algorithms. We use 3 datasets (200k samples each) with different qualities from the Hopper task: \underline{hopper-random} from a randomly initialized policy, \underline{hopper-medium} from a policy trained to approximately 1/3 the performance of a policy trained to completion with SAC ("expert"), and \underline{hopper-medium-expert} from a 50-50 split of medium and expert data.

\begin{figure*}[t]%
\vspace{-2em}
    \centering
    \includegraphics[width=\linewidth]{images/combined_sepsis.pdf}
    \caption{\looseness=-1\textbf{(a)} We first compare our proposed pipeline to various other policy selection approaches in the Sepsis POMDP task. Our approach \ssr-RRS 5-split consistently obtains policies that on average perform close to the optimal policy, significantly outperforming other approaches. \textbf{(b)} We investigate the importance of re-training in the small (N=200) to medium (N=1000) data regime. We show the true reward obtained by all policies from all \ah pairs either trained on 50\% of the data or 100\% of the data. 95\% confidence intervals are depicted as error bars. Most policies achieve higher rewards when trained on more data, even more so when the dataset is small or when tasks are more difficult (Robomimic).}
    \vspace{-1em}
    \label{fig:fig2}
\end{figure*}

\subsection{Baselines}

\textbf{One-Split OPE.} %
\looseness=-1 The simplest method to train and verify an algorithm's performance without access to any simulator is to split the data into a train $\train$ and valid set $\valid$. All policies are trained on the same training set and evaluated on the same valid set. As we explained before, this method has the high potential of overfitting the chosen hyperparameter for one data partition -- it might pick the best policy, but does not guarantee we can use the same hyperparameter to re-train on the full dataset.



\textbf{OPE on Bootstrapped Val.}
Bootstrapping is a popular re-sampling technique that estimates prediction error in supervised learning models~\citep{efron1983estimating,efron1986biased}. The idea of using bootstrapping for OPE estimate is first utilized in HCOPE \citep{thomas2015high}.
Compared to the one-split method and the \ssr pipeline, bootstrapping trains all policies on the same training dataset, and only considers variations in the validation set by creating bootstrapped samples. We refer to the considered Bias-corrected accelerated (BCa) bootstrap method as \textbf{BCa} in the experiments.

\textbf{Cross-Validation (CV).}
One other natural alternative of repeated experiment validation is the popular M-fold Cross-Validation method~\citep{stone1974cross}.
M-fold CV constructs a non-overlapping set of trajectories from the original dataset. For example, a 5-fold CV will train a policy on 80\% of data and evaluate the policy on 20\% of data, as it divides the dataset into 5 non-overlapping partitions.
However, as  we increase the number of splits $M$, which allows us to train/test our algorithms under more data split variations, each non-overlapping set $\mathcal{D}_m$ becomes smaller. When $M=n-1$, M-fold CV becomes leave-one-out CV (LooCV). In this extreme case, many OPE estimators will not work properly, as we have shown in Appendix~\ref{ap:proof}.
We further investigate a variant of M-fold CV called Nested M-fold CV (\textbf{Nested CV}), 
which repeats the M-fold non-overlapping partitioning K times. This procedure is computationally very expensive. Considering the fairness of comparison and computational efficiency, we only evaluate $K \times 2$-fold CV.

\textbf{OPE with BVFT.} Batch Value Function Tournament is the closest competitor to our method, which is a meta-algorithm for hyperparameter-free policy selection~\citep{xie2021batch,zhang2021towards}. For a set of Q-value functions, BVFT makes pairwise comparisons of each (tournament-style) to select the best out of the entire set based on the BVFT-Loss.
Compared to our method, BVFT incurs $\mathcal{O}(J^2)$ comparison given $J$ \ah pairs, practically infeasible for large $J$. The original BVFT can only compare Q-functions, therefore only usable with OPL that directly learns Q-functions. \cite{zhang2021towards} offers an extension to BVFT by using BVFT to compare between FQEs, therefore allowing BVFT to be OPL-agnostic. We adopt the two strategies recommended by the paper. Given $J$ \ah pairs and $B$ FQEs, strategy 1 compares $J \times B$ FQE's Q-functions jointly (\textbf{$\pi$ x FQE}) and strategy 2 compares $B$ FQEs within each \ah and pick the best FQE as the estimate of the \ah's value estimate (\textbf{$\pi$ + FQE}). 
We discuss more in Appendix~\ref{ap:alternative_approaches} (calculations) and \ref{ap:comp_complexity} (time complexity).




\subsection{Training and Evaluation} %
\textbf{Offline Policy Learning.} 
In the following, we outline a variety of Offline RL algorithms used in the evaluation of the \ssr pipeline to demonstrate the generality of our approach and that it can reliably produce the optimal final policy using the selected \ah pair. This marks a departure from workflows designed for specific algorithms, such as~\citet{kumar2021a}. We experiment with popular offline RL methods (see Table~\ref{tab:algs} and we provide algorithmic and hyperparameter details in Table~\ref{tab:domain-details}).
\textbf{Offline Policy Evaluation.}
We use WIS estimators for the tabular and discrete action domains: Sepsis and TutorBot. We use FQE for continuous action domains: Robomimic and D4RL. For each task, with a given dataset, we use the splitting procedure described in Section~\ref{sec:approach} to generate the partitioning. We describe how we compute the results for each figure in Appendix~\ref{ap:figgen}.



\begin{table*}[]
\small
\centering 
\begin{tabular}{@{}rlc@{}}
\toprule
Category                   & \multicolumn{1}{c}{Algorithms}                                         & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Internal \\ Q-function\end{tabular}} \\ \midrule
Imitation Learning         & \begin{tabular}[c]{@{}l@{}}BC~\citep{pomerleau1991efficient}\\ BCRNN~\citep{mandlekar2018roboturk}\end{tabular}                     & \xmark                                                                             \\
Conservative Model-Free    & \begin{tabular}[c]{@{}l@{}}BCQ~\citep{fujimoto2019off}, CQL~\citep{kumar2020conservative}, \\ IRIS~\citep{mandlekar2020iris}\end{tabular}              & \cmark                                                                             \\
Policy Gradient & \begin{tabular}[c]{@{}l@{}}POIS~\citep{metelli2018policy}, BC+POIS (ours), BC+mini-POIS (ours)\end{tabular} & \xmark                                                                             \\
Offline Model-Based        & \begin{tabular}[c]{@{}l@{}}MOPO~\citep{yu2020mopo}, P-MDP (ours)\end{tabular}                 & \cmark                                                                             \\ \bottomrule
\end{tabular}
\caption{List of \ah we are comparing in our experiments.}
\label{tab:algs}
\end{table*}









\begin{figure*}[t]%
    \centering
    \includegraphics[width=\linewidth]{images/combined_heatmap_datasize.pdf}
    \caption{\textbf{(a)} We show the effect of choosing $K$ (the number of train/valid splits) for \ssr-RRS. We ablate $K$ and run the simulation 500 times. The heatmaps shows the frequency at which each policy is chosen by our method and its final performance in the environment. In this experiment, \ssr-RRS chooses over 540 \ah pairs. As we can see, when the number of splits $K$ is larger, \ssr-RRS consistently pick better policies. \textbf{(b)} In the Sepsis-POMDP domain, we show that as the number of trajectories ($N$) in the offline dataset increases, data partitioning becomes less important. Though RRS still outperforms the 1-split policy selection.} %
    \vspace{-1em}
    \label{fig:heatmap_benefit_split}
\end{figure*}











==> fvcxkgstnhxcyccfvtcknzrmdvqdfdgy_arXiv/intro.tex <==
\section{Introduction}
\label{sec:intro}

Offline/batch reinforcement learning has the potential to learn better decision policies from existing real-world datasets on sequences of decisions made and their outcomes. In many of these settings, tuning methods online is infeasible and deploying a new policy involves time, effort and potential negative impact. Many of the  existing datasets for applications that may benefit from offline RL may be fairly small in comparison to supervised machine learning. For instance, the MIMIC intensive care unit dataset on sepsis that is  often studied in offline RL has 14k patients~\citep{komorowski2018artificial}, the number of students frequently interacting with an online course will often range from hundreds to tens of thousands~\citep{bassen2020reinforcement}, and the number of demonstrations collected from a human operator manipulating a robotic arm is often on the order of a few hundred per task~\citep{mandlekar2018roboturk}. In these small data regimes, recent studies~\citep{mandlekar2021what,levine2020offline} highlight that with limited data, the selection of hyperparameters using the training set is often challenging. Yet hyperparameter selection also has a  substantial influence on the resulting policy's performance, particularly when the algorithm leverages deep neural networks.



One popular approach to address this is to learn policies from particular algorithm-hyperparameter pairs on a training set and then use offline policy selection, which selects the best policy given a validation set~\citep{pmlr-v37-thomas15,thomas2019preventing,paine2020hyperparameter,kumar2021a}. %
However, when the dataset is limited in size, this approach can be limited: (a) if the validation set happens to have no or very few good/high-reward trajectories, then trained policies cannot be properly evaluated; (b) if the training set has no or very few such trajectories, then no good policy behavior can be learned through any policy learning algorithm; and (c) using one fixed training dataset is prone to overfitting the hyperparameters on this one dataset and different hyperparameters could be picked if the training set changes. One natural solution to this problem is to train on the entire dataset and compare policy performance on the same dataset, which is often referred to as the internal objective approach. In  Appendix~\ref{ap:prelude} we conduct a short experiment using D4RL where this approach fails due to the common issue of Q-value over-estimation~\citep{fujimoto2019off}.%




There has been much recent interest in providing more robust methods for offline RL. Many rely on the  workflow just discussed, where methods are trained on one dataset and 
Offline Policy Evaluation (OPE) is used to do policy selection~\citep{su2020adaptive,paine2020hyperparameter,zhang2021towards,kumar2021a,lee2021model,tang2021model,miyaguchi2022theoretical}. Our work highlights the impact of a less studied issue: the challenge caused by data partitioning variance. We first motivate the need to account for train/validation partition randomness by showing the wide distribution of OPE scores the same policy can obtain on different subsets of data or the very different performing policies the same algorithm and hyperparameters can learn depending on different training set partitions. We also prove a single partition can have a notable failure rate in identifying the best algorithm-hyperparameter to learn the best policy. 





We then introduce a general pipeline for algorithm-hyperparameters (\ah) selection and policy deployment that: (a) uses repeated random sub-sampling (RRS) with replacement of the dataset to perform \ah training, (b) uses OPE on the validation set, (c) computes aggregate statistics over the RRS splits to inform \ah selection, and (d) allows to use the selected \ah to retrain on the entire dataset to obtain the deployment policy. Though such repeated splitting is common in supervised learning, its impact and effect have been little studied in the offline RL framework. Perhaps surprisingly, we show that our simple pipeline leads to substantial performance improvements in a wide range of popular benchmark tasks, including D4RL~\citep{fu2020d4rl} and Robomimic~\citep{mandlekar2021what}. 










==> fvcxkgstnhxcyccfvtcknzrmdvqdfdgy_arXiv/math_commands.tex <==

\usepackage{amsmath,amsfonts,bm}

\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

\newcommand{\newterm}[1]{{\bf #1}}


\def\figref#1{figure~\ref{#1}}
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
\def\secref#1{section~\ref{#1}}
\def\Secref#1{Section~\ref{#1}}
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
\def\eqref#1{equation~\ref{#1}}
\def\Eqref#1{Equation~\ref{#1}}
\def\plaineqref#1{\ref{#1}}
\def\chapref#1{chapter~\ref{#1}}
\def\Chapref#1{Chapter~\ref{#1}}
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
\def\algref#1{algorithm~\ref{#1}}
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
\def\partref#1{part~\ref{#1}}
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\data}{\mathcal{D}}
\newcommand{\train}{\mathcal{D_{\mathrm{train}}}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}



\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

\newcommand{\pdata}{p_{\rm{data}}}
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} %

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} %

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> fvcxkgstnhxcyccfvtcknzrmdvqdfdgy_arXiv/method.tex <==

\section{\ssr: Repeated Random Sampling for $\gA_i$ Selection and Deployment}
\label{sec:approach}
\vspace{-3mm}







\looseness=-1 In this paper, we are interested in the following problem: \textit{If offline RL training and evaluation are very sensitive to the partitioning of the dataset, especially in small data regimes, how can we reliably produce a final policy that we are confident is better than others and can be reliably deployed in the real-world?}\\
Instead of considering the sensitivity to data partition as an inherent obstacle for offline policy selection, we view this as statistics to leverage for \emph{$\gA_i$} selection.
We propose a general pipeline: \textit{Split Select Retrain} (\ssr) (of which we provide a pseudo-code in Algorithm~\ref{alg:ssr-rs}, Appendix~\ref{ap:alg}) to reliably optimize for a good deployed policy given only: an offline dataset, an input set of \ah pairs and an off-policy evaluation (OPE) estimator. 
This deployment approach leverages the random variations created by dataset partitioning to select algorithms that perform better \emph{on average} using a robust hyperparameter evaluation approach which we develop below.

First, we split and create different partitions of the input dataset. For each train/validation split, each algorithm-hyperparameter (\ah) is trained on the training set and evaluated using the input OPE method to yield an estimated value on the validation set. These estimated evaluations are then averaged, and the best \ah pair ($\gA^*$) is selected as the one with the highest average score. Now the last step of the \ssr pipeline is to re-use the entire dataset to train one policy $\pi^*$ using $\gA^*$.
 
 








\paragraph{Repeated Random Sub-sampling (RRS).}
As Theorem~\ref{thm:benefit_n_splits} suggests, one should ensure a sufficient amount of trajectories in the evaluation partition to lower the failure rate $C$. We propose to create RRS train-validation partitions. 
This approach has many names in the statistical model selection literature, such as Predictive Sample Reuse Method~\citep{geisser1975predictive}, Repeated Learning-Test Method~\citep{burman1989comparative} or Monte-Carlo Cross-Validation~\citep{dubitzky2007fundamentals}. It has also been referred to as Repeated Data Splitting~\citep{chernozhukov2018generic} in the heterogeneous treatment effect literature.\\
We randomly select trajectories in $\data$ and put them into into two parts: $R^{\mathrm{train}}$ and $R^{\mathrm{valid}}$. We repeat this splitting process $K$ times to generate paired datasets: $(R^{\mathrm{train}}_1, R^{\mathrm{valid}}_1), (R^{\mathrm{train}}_2, R^{\mathrm{valid}}_2), ..., (R^{\mathrm{train}}_K, R^{\mathrm{valid}}_K)$. We compute the generalization performance estimate as follows:
\begin{align}
    \gG_{\mathcal{A},\mathrm{RS}_K} = \frac{1}{K} \sum_{k=1}^K \big [\hat V(\mathcal{A}(R^\mathrm{train}_k); R^\mathrm{valid}_k) \big ]
\end{align}

\looseness=-1 A key advantage of overlap partitioning is that it maintains the size of the validation  dataset as $K$ increases. This might be favorable since OPE estimates are highly dependent on the  state-action coverage of the validation dataset -- the more data in the validation  dataset, the better OPE estimators can evaluate a policy's performance. As $K \rightarrow \infty$, RRS approaches the leave-$p$-out cross-validation (CV), where $p$ denotes the number of examples in the validation dataset.
Since there are $\binom{n}{p}$ possible selections of $p$ data points out of $n$ in our dataset, it is infeasible to use exact leave-$p$-out CV when $p > 2$, but a finite $K$ can still offer many advantages. Indeed,~\citet{krzanowski1997assessing} point out that leave-$p$-out estimators will have lower variance compared to leave-one-out estimators, which is what the more commonly used M-fold cross-validation method converges to when $M = n-1$. We discuss more in Appendix~\ref{ap:leave-p-out}.

















==> fvcxkgstnhxcyccfvtcknzrmdvqdfdgy_arXiv/notations.tex <==
\newcommand{\treeroot}{\varnothing}
\newcommand{\transitiondescriptor}{P}
\newcommand{\transitionkernel}[1]{P_{#1}}
\newcommand{\rewarddescriptor}{R}
\newcommand{\rewardkernel}[1]{R_{#1}}
\newcommand{\history}{\eta}

\newcommand{\ith}[1]{#1^{(i)}}
\newcommand{\Wsum}{W}

\newcommand{\wis}{\hat{v}_{\text{SNIS}}}
\newcommand{\tis}{\hat{v}_{\text{TIS}}}
\newcommand{\wtis}{\hat{v}_{\text{SNTIS}}}
\newcommand{\Dcal}{\mathcal{D}}
\newcommand{\Bcal}{\mathcal{B}}
\newcommand{\empE}{\hat{\EE}}

\newcommand{\Aset}{A}
\newcommand{\dist}{\mathrm{dist}}
\newcommand{\threshold}{\delta}

\newcommand{\Prob}{\mathrm{P}}
\newcommand{\ispg}{\textsc{POELA}\xspace}
\newcommand{\ispgbaseline}{PO-CRM\xspace}
\newcommand{\ispgknn}{PO-$\mu$}
\newcommand{\ispgmuhat}{PO-$\hat{\mu}$}

\newtheorem{example}{Example}


==> fvcxkgstnhxcyccfvtcknzrmdvqdfdgy_arXiv/offline_alg.tex <==

\begin{figure*}[t]%
\vspace{-2em}
    \centering
    \includegraphics[width=\linewidth]{images/Figure0_wide.pdf}
    \caption{\looseness=-1True performance and evaluation of 6 $\mathcal{A}_i$ pairs on the Sepsis-POMDP (N=1000) domain. (a) shows the OPE estimations and (b) shows the variation in terms of true performance. The variations are due to the different \ah pairs of the policies \textit{but also} to the sensitivity to the training/validation splits.%
    }
    \label{fig:new-variation}
\end{figure*}



\section{The Challenge of Offline RL $\mathcal{A}_i$ Selection}
\label{sec:offline}
An interesting use-case of offline RL is when domain experts have access to an existing dataset (with potentially only a few hundred trajectories) about sequences of decisions made and respective outcomes, with the hope of leveraging the dataset to learn a better decision policy for future use. In this setting, the user may want to consider many options regarding the type of RL algorithm (model-based, model-free, or direct policy search), hyperparameter, or deep network architecture to use.






Automated algorithm selection is important because different $\mathcal{A}_i$ (different \ah pairs) may learn very diverse policies, each with significantly different performance $V^{\mathcal{A}_i}$. Naturally, one can expect that various algorithms lead to diverse performance, but using a case-study experiment on a sepsis simulator~\citep{oberst2019counterfactual}, we observe in Figure~\ref{fig:new-variation}(b) that the sensitivity to hyperparameter selection is also substantial (cf. different average values in box plots for each method). For example, MBS-QI~\citep{liu2020provably} learns policies ranging from over -12 to -3 in their performance, depending on the hyperparameters chosen.







Precisely, to address hyperparameter tuning, past work often relies on executing the learned policies in the  simulator/real environment. When this is not feasible, as in many real-world applications, including our sepsis dataset example, where the user may only be able to leverage existing historical data, we have no choice but to rely on off-policy evaluation. Prior work~\citep{thomas2015high,farajtabar2018more,thomas2019preventing,mandlekar2021what} have suggested doing so using a hold-out method, after partitioning the dataset into training and validation sets.

Unfortunately, the partitioning of the dataset itself may result in substantial variability in the training process~\citep{dietterich1998approximate}. We note that this problem is particularly prominent in offline RL where high-reward trajectories are sparse and affect both policy learning and policy evaluation. To explore this hypothesis, we consider the influence of the train/validation partition in the same sepsis domain, and we evaluate the trained policies using the Weighted Importance Sampling (WIS)~\citep{precup2000eligibility} estimator. Figure~\ref{fig:new-variation}(a) shows the policies have drastically different OPE estimations with sensitivity to randomness in the dataset partitioning. We can observe the same phenomena in Figure~\ref{fig:new-variation}(b) with largely different true performances depending on the dataset splitting for most of the policies $\mathcal{A}_i$. This is also illustrated on the left sub-figure of Figure~\ref{fig:heatmap_benefit_split} where in the case where a single train-validation split is used, an $\mathcal{A}_i$ that yields lower-performing policies will often be selected over those that yield higher-performing policies when deployed.















\subsection{Repeated Experiments for Robust Hyperparameter Evaluation in Offline RL}
\label{sec:theory}
We now demonstrate why it is important to conduct repeated random sub-sampling on the dataset in offline RL. Consider a finite set of $J$ offline RL algorithms $\mathcal{A}$. Let the policy produced by algorithm $\mathcal{A}_j$ on training dataset $\mathcal{D}$ be $\pi_j$, its estimated performance on a validation set $\hat{V}^{\pi_j}$, and its true (unknown) value be $V^{\pi_j}.$ Denote the true best resulting policy as $\pi_{j^*} = \argmax_j V^{\pi_j}$ and the corresponding algorithm $\mathcal{A}_{j^*}$. Let the best policy picked based on its validation set performance as $\pi_{\hat{j}^*} = \argmax_j \hat{V}^{\pi_j}$ and the corresponding algorithm $\mathcal{A}_{\hat{j}^*}$. 
\begin{theorem}
\label{thm:benefit_n_splits} 
There exist stochastic decision processes and datasets such that (i) using a single train/validation split procedure that selects an algorithm-hyperparameter with the best performance on the validation dataset will select a suboptimal policy and algorithm with significant finite probability, $P(\pi_{\hat{j}^*} \neq \pi_{j^*}) \geq C$, with corresponding substantial loss in performance $O(V_{max})$, and, in contrast,  (ii) selecting the algorithm-hyperparameter with the best average validation performance across $N_s$ train/validation splits will select the optimal algorithm and policy with probability 1: $\lim_{N_s\to\infty} P(\pi_{\hat{j}^*} = \pi_{j^*}) \to 1.$
\end{theorem}
\textit{Proof Sketch.} Due to space constraints we defer the proof to Appendix~\ref{ap:proof}. Briefly, the proof proceeds by proof by example through constructing a chain-like stochastic decision process and considers a class of algorithms that optimize over differing horizons (see e.g.~\cite{jiang2015dependence,cheng2021heuristic,mazoure2021improving}). The behavior policy is uniformly random meaning that trajectories with high rewards are sparse. This means there is a notable probability that in a single partition of the dataset, the  resulting train and/or validation set may not contain a high reward trajectory, making it impossible to identify that a full horizon algorithm, and resulting policy, is optimal. 


In the proof and our experiments, we focus on when the training and validation sets are of equal size. If we use an uneven split, such as $80/20\%$, the failure probability can further increase if only a single partition of the dataset is used. We provide an illustrative example in the Appendix. 
Note that Leave-one-out Cross-Validation (LooCV) will also fail in our setting if we employ, as we do in our algorithm, WIS, because as a biased estimator, WIS will return \textit{the observed return of the behavior policy if averaging over a single trajectory, independent of the target policy to be evaluated}. We explain this further in Appendix~\ref{ap:add-discussion}.






==> fvcxkgstnhxcyccfvtcknzrmdvqdfdgy_arXiv/problem_new.tex <==

\section{Background and Problem Setting}
\label{sec:problem}
We define a stochastic Decision Process $M =$ $\langle \gS, A, T, r, \gamma \rangle$, where $\gS$ is a set of states; $A$ is a set of actions; $T$
is the transition dynamics (which might depend on the full history); $r$
is the reward function; and $\gamma \in (0, 1)$ is the discount factor. Let $\tau = \{s_i, a_i, s_i', r_i\}_{i=0}^L$ be the trajectory sampled from $\pi$ on $M$. The optimal policy $\pi$ is the one that 
maximizes the expected discounted return $V(\pi) = \E_{\tau \sim  \rho_\pi}[G(\tau)]$ where $G(\tau) = \sum_{t=0}^{\infty} \gamma^t r_t$ and $\rho_\pi$ is the distribution of $\tau$ under policy $\pi$.
For simplicity, in this paper we assume policies are Markov $\pi: S \rightarrow A$, but it is straightforward to consider policies that are a function of the full history. In an offline RL problem, we take a dataset: $\data = \{\tau_i\}_{i=1}^n$, which can be collected by one or a group of policies which we refer to as the behavior policy $\pi_b$ on the decision process $M$. The goal in offline/batch RL is to learn a decision policy $\pi$ from a class of policies with the best expected performance $V^{\pi}$ for future use. 
Let $\mathcal{A}_i$ to denote an \ah pair, i.e. an offline policy learning algorithm and its hyperparameters and model architecture. %
An offline policy estimator takes in a policy $\pi_e$ and a dataset $\data$, and returns an estimate of its performance: $\widehat V: \Pi \times \data \rightarrow \R$. In this work, we focus on two popular Offline Policy Evaluation (OPE) estimators: Importance Sampling (IS)~\citep{precup2000eligibility} and Fitted Q-Evaluation (FQE)~\citep{le2019batch} estimators. We refer the reader to \cite{voloshin2021empirical} for a more comprehensive discussion.



==> fvcxkgstnhxcyccfvtcknzrmdvqdfdgy_arXiv/pseudocode.tex <==
\begin{algorithm}[t]
\SetAlgoLined
\SetKwFunction{subsample}{Subsample}
\SetKwFunction{append}{append}
\KwIn{offline RL data $\data$; A set of AH pairs [$\gA_1, \gA_2, ..., \gA_z$], an OPE estimator  $\widehat V$, and choose a split number $K\in \mathbb{N}$.}
\KwOut{policy $\hat \pi^*$ for deployment}
\BlankLine
$\gR$ = []  \Comment{\textcolor{red}{The split step}}\\
\For{$i \leftarrow 1...K$}{
    $R^\mathrm{train}_i, R^\mathrm{valid}_i = $ \subsample($\data, 0.5$)
    $\gR = \gR \cup (R^\mathrm{train}_i, R^\mathrm{valid}_i)$
}
$\gG$ = []  \Comment{\textcolor{red}{The select step}}\\
\For{$i \leftarrow 1...z$}{
    $\gS$ = [] \\
    \For{$j \leftarrow 1...K$}{
        $\pi_i = \mathcal{A}(R^\mathrm{train}_j)$ \\
        $\theta_j = \widehat V(\pi_i; R^\mathrm{valid}_j)$ \\
        $\gS = \gS \cup \theta_j$ \\
     }
     $\gG = \gG \cup \frac{1}{K} \sum_{j=1}^K \gS_j$ \Comment{\small{\textcolor{red}{One score per algorithm}}}
 }
  $\gA^* = \gA_{o+}$ where $o = \argmax(\gG)$ \Comment{\small{\textcolor{red}{Choose the highest}}}\\
 $\pi^* = \gA^*(\data)$ \Comment{\textcolor{red}{The full retrain step}} \\
 \Return{$\pi^*$}
 \caption{Split-Select-Retrain with Repeated Random Sub-sampling (SSR-RS)}
 \label{alg:ssr-rs}
\end{algorithm}

==> fvcxkgstnhxcyccfvtcknzrmdvqdfdgy_arXiv/related.tex <==





\begin{table*}[t]
\small
\centering
\begin{tabular}{@{}rccccc@{}}
\toprule
Common Practices                                                                                      & \begin{tabular}[c]{@{}c@{}}Non-Markov \\ Env\end{tabular}  & \begin{tabular}[c]{@{}c@{}}Data \\ Efficient\\(re-train)\end{tabular} & \begin{tabular}[c]{@{}c@{}}Compare \\ Across \\ OPL\end{tabular} & \begin{tabular}[c]{@{}c@{}}Considers \\ Evaluation \\ Variation\end{tabular} & \begin{tabular}[c]{@{}c@{}}Considers \\ Training \\ Variation\end{tabular} \\ \midrule
\multicolumn{6}{l}{\textbf{Policy selection (1 split)}}                                                                                                                                                                                                                                                                                                                                                \\ \midrule
\begin{tabular}[c]{@{}r@{}}Internal Objective / TD-Error\\\citep{thomas2015high,thomas2019preventing}\end{tabular}      & (depends)  &   \xmark                                                        &   \xmark                                                               &   \xmark                                                                           &     \xmark                                                                       \\ \midrule
OPE methods \\ (\cite{komorowski2018artificial};\\\cite{paine2020hyperparameter}                                                                                           &    (depends)                   &   \xmark                                                        &      \cmark                                                            &      \xmark                                                                        &         \xmark                                                                   \\ \midrule
\begin{tabular}[c]{@{}r@{}}OPE + BCa Val. \\\citep{thomas2015high}\end{tabular}                              &  (depends)                                                            &    \xmark                                                       &    \cmark                                                              &     \cmark                                                                         &     \xmark                                                                       \\ \midrule
\begin{tabular}[c]{@{}r@{}} BVFT \\\citep{xie2021batch} \end{tabular}              &  \xmark                                         &   \xmark                                      &  \xmark                                             &  \xmark                                                        &  \xmark                                                       \\ \midrule
\begin{tabular}[c]{@{}r@{}}BVFT + OPE \\\citep{zhang2021towards}\end{tabular}                                                              &      \xmark                     &   \xmark                                                                &    \cmark                                                                          &     \cmark       &  \xmark                                                                 \\ \midrule
\begin{tabular}[c]{@{}r@{}}Q-Function Workflow \\ \citep{kumar2021a}  \end{tabular}                                                                                        &  \xmark                                                             & \cmark                                                          &  \xmark                                                                &    \xmark                                                                          &          \xmark                                                                  \\ \midrule
\multicolumn{6}{l}{\textbf{Ours: $\gA_i$ selection (multi-split)}}                                                                                                                                                                       \\ \midrule
Cross-Validation                                                                            & \cmark                                       & \cmark & \cmark                                      & \cmark                                             & \cmark                                                                                                         \\ \midrule
\begin{tabular}[c]{@{}r@{}}Repeated Random \\ Subsampling\end{tabular}                  & \cmark                                       & \cmark & \cmark                                      & \cmark                                             & \cmark                                                                                                             \\ \bottomrule
\end{tabular}
\caption{A summary of commonly used approaches for choosing a deployment policy from a fixed offline RL dataset. We define \textit{Data Efficient} as: the approach assumes the algorithm can be re-trained on all data points; \textit{(depends)} as: depends on whether the underlying OPL or OPE methods make explicit Markov assumption or not.}
\label{tab:ops}

\end{table*}

\section{Related work}



\looseness=-1\textbf{Offline Policy Learning (OPL).}
In OPL, the goal is to use historical data from a fixed behavior policy $\pi_b$ to learn a reward-maximizing policy in an unknown environment (Markov Decision Process, defined in Section~\ref{sec:problem}).
Most work studying the sampling complexity and efficiency of offline RL~\citep{xie2021batch,yin2021near} do not depend on the structure of a particular problem, but empirical performance may vary with some pathological models that are not necessarily Markovian.~\citet{shi2020does} have precisely developed a model selection procedure for testing the Markovian hypothesis and help explain different performance on different models and MDPs.
To address this problem, it is inherently important to have a fully adaptive characterization in RL because it could save considerable time in designing domain-specific RL solutions~\citep{zanette2019tighter}.
As an answer to a variety of problems, OPL is rich with many different methods ranging from policy gradient~\citep{DBLP:conf/uai/LiuSAB19}, model-based~\citep{yu2020mopo,kidambi2020morel}, to model-free methods~\citep{Siegel2020Keep,fujimoto2019off,guo2020batch,kumar2020conservative} each based on different assumptions on the system dynamics. Practitioners thus dispose of an array of algorithms and corresponding hyperparameters with no clear consensus on a generally applicable evaluation tool for offline policy selection.

\textbf{Offline Policy Evaluation (OPE).}
OPE is concerned with evaluating a target policy's performance using only pre-collected historical data generated by other (behavior) policies~\citep{voloshin2021empirical}. Each of the many OPE estimators has its unique properties, and in this work, we primarily consider two main variants~\citep{voloshin2021empirical}: Weighted Importance Sampling (WIS)~\citep{precup2000eligibility} and Fitted Q-Evaluation (FQE)~\citep{le2019batch}. Both WIS and FQE are sensitive to the partitioning of the evaluation dataset. WIS is undefined on trajectories where the target policy does not overlap with the behavior policy and self-normalizes with respect to other trajectories in the dataset. FQE learns a Q-function using the evaluation dataset. This makes these estimators very different from mean-squared errors or accuracy in the supervised learning setting -- the choice of partitioning will first affect the function approximation in the estimator and then cascade down to the scores they produce.

\textbf{Offline Policy Selection (OPS).}
Typically, OPS is approached via OPE, which estimates the expected return of candidate policies.~\citet{zhang2021towards} address how to improve policy selection in the offline RL setting. The algorithm builds on the Batch Value-Function Tournament (BVFT)~\citep{xie2021batch} approach to estimating the best value function among a set of candidates using piece-wise linear value function approximations and selecting the policy with the smallest projected Bellman error in that space. Previous work on estimator selection for the design of OPE methods include~\citet{su2020adaptive,miyaguchi2022theoretical} while ~\citet{kumar2021a,lee2021model,tang2021model,paine2020hyperparameter} focus on offline hyperparameter tuning.~\citet{kumar2021a} give recommendations on when to stop training a model to avoid overfitting. The approach is exclusively designed for Q-learning methods with direct access to the internal Q-functions. On the contrary, our pipeline does policy training, selection, and deployment on any offline RL method, not reliant on the Markov assumption, and can select the best policy with potentially no access to the internal approximation functions (black box). We give a brief overview of some OPS approaches in Table~\ref{tab:ops}.








==> fvcxkgstnhxcyccfvtcknzrmdvqdfdgy_arXiv/result.tex <==

\section{Results}
\label{sec:results}



\begin{table*}[ht!]
\centering
\small
\begin{tabular}{rccccccc}
\toprule
\begin{tabular}[c]{@{}r@{}}Re-trained\\ on full dataset\end{tabular} & \begin{tabular}[c]{@{}c@{}}BVFT-FQE\\ $\pi$ x FQE\end{tabular} & \begin{tabular}[c]{@{}c@{}}BVFT-FQE\\ $\pi$ + FQE\end{tabular} & \begin{tabular}[c]{@{}c@{}} CV-2\end{tabular} & \begin{tabular}[c]{@{}c@{}} CV-5\end{tabular} & \begin{tabular}[c]{@{}c@{}}\ssr\\ RRS-2\end{tabular} & \begin{tabular}[c]{@{}c@{}}\ssr\\ RRS-5\end{tabular} & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Optimal\\ Policy\end{tabular}} \\ \midrule
\multicolumn{1}{l}{\textbf{Robomimic:}} &  &  &  &  &  &  &  \\
Can-Paired & \multicolumn{1}{c}{0.65} & \multicolumn{1}{c}{{0.71}} & \multicolumn{1}{c}{{0.72}} & \multicolumn{1}{c}{{0.72}} & \multicolumn{1}{c}{{0.71}} & \multicolumn{1}{c}{\textbf{0.73}} & \multicolumn{1}{c}{0.75} \\
Transport & \multicolumn{1}{c}{0.21} & \multicolumn{1}{c}{0.0} & \multicolumn{1}{c}{0.42} & \multicolumn{1}{c}{0.42} & \multicolumn{1}{c}{0.62} & \multicolumn{1}{c}{\textbf{0.70}} & \multicolumn{1}{c}{0.74} \\ \midrule
\multicolumn{1}{l}{\textbf{D4RL (Hopper):}} &  &  &  &  &  &  &  \\
random & 321.75 & 317.72 & \textbf{325.37} & \textbf{325.37} & 324.92 & \textbf{325.37} & 325.37 \\
medium & 934.71 & 1227.81 & 1227.81 & 1304.53 & 1296.87 & \textbf{1304.54} & 1392.93 \\
medium-expert & 2677.93 & 2677.93  & 2530.04 & 2530.04 & 3481.34 & \textbf{3657.80} & 3657.80 \\ \midrule
\multicolumn{1}{l}{\textbf{Sepsis:}} &  &  &  &  &  &  &  \\
MDP (n=200) & --- & -19.32  & -10.26 & -20.32 & -13.01 & \textbf{-7.85} & -1.94 \\
POMDP (n=1000) & ---  & -1.92 & 0.74 & -1.92 & 2.40 & \textbf{6.75} & 7.86 \\ \midrule
\multicolumn{1}{l}{\textbf{TutorBot:}} &  &  &  &  &  &  &  \\
POMDP (n=200) & ---  & ---  & 1.34 & 1.19 & 1.30 & \textbf{1.38} & 1.43 \\ \bottomrule
\end{tabular}
\caption{Comparison of the performance obtained by a policy deployed using the \ssr pipeline vs. using 1-split policy selection approaches on a wide range of application domains. Cells = average true return. We note that ($\pi$ x FQE) is very computationally expensive when we search through a large \ah space (in Sepsis and TutorBot), therefore we exclude them.}
\label{tab:alldomains}
\vspace{-2mm}
\end{table*}




\textbf{$\mathcal{A}_i$ Selection Comparison.}
In Figure~\ref{fig:fig2}(a), we compare five approaches (One-Split OPE, BCa, BVFT-FQE, CV, and \ssrrrs) on the Sepsis-POMDP domain with 1000 patients. For each approach, we compute a score per \ah pair, and select the best algorithm according to each. For fairness in comparison, all selected $\mathcal{A}_i$ are re-trained on the full dataset and we report the final performance in the real environment. As expected, \textbf{One-Split OPE} performed the worst. Surprisingly, using the lower bound of bootstrapped (\textbf{BCa (LB)}) confidence interval also does not allow to pick good policies, LB being perhaps too conservative. We see that \textbf{CV 2-fold} and \textbf{CV 5-fold} do not perform well either. \textbf{CV 2-fold} does not allow enough repetition and \textbf{CV 5-fold} makes the validation set size too small.
We observe clearly that \textbf{\ssrrrs 5-split} performs the best and selected policies that are on average very close to the optimal policy's performance.
\textbf{BVFT-FQE} relies on FQE, which is a misspecified model on the Sepsis domain and difficult to optimize given the small dataset size; hence it does not select good policies in Sepsis. However, in Robomimic Can-Paired and D4RL Hopper, BVFT-FQE is able to pick good policies, albeit not significantly better or worse than other methods, and still worse than \textbf{\ssrrrs 5-split} in the mixed (more realistic) “medium-expert” dataset. We show more analysis of BVFT compared to our method in the Appendix.
Table~\ref{tab:alldomains} aggregates the results for all the considered domains in our study. Our approach \textbf{\ssrrrs 5-split} is distinctly able to more consistently select policies that, once deployed, perform close to the optimal policy across all tasks.

\textbf{The Benefits of Re-training Policies Selected with \ssr.}
In Figure~\ref{fig:fig2}(b), we plot the true reward of a selected policy $\mathcal{A}_i$ when only trained on 50\% of the dataset (the training set) compared to when trained on 100\% of the dataset. As expected, in the small data regime, every single trajectory matters. Policies trained on the full dataset significantly outperform policies trained only on half of it. This experiment provides strong evidence in favor of \ah selection (done with RRS on the full dataset) over policy selection (done on the training set) in offline RL.

\textbf{The Impact of Number of Repeats for \ssrrrs.}
The proposed pipeline \ssrrrs has a hyperparameter $K$ for the number of repeated data splitting. In Figure~\ref{fig:heatmap_benefit_split}(a), we show the true performance of the policy that is being selected by \textbf{\ssrrrs} with $K=1,2,5$ by running 500 simulations with heatmaps on the frequency of each policy is selected. We observe that when $K=1$ (equivalent to the One-Split OPE method), policies are picked quite uniformly; many of which are performing poorly. When $K=5$, higher-performing policies are selected much more frequently. From Table~\ref{tab:alldomains}, we conclude that $K=5$ generally works well across various domains. Naturally, the number of split $K$ will be chosen in line with the computing budget available; $K=5$ appears to be a reasonable choice.


\textbf{The Impact of Dataset Size.}
\looseness=-1 Finally, we investigate to which extent the proposed pipeline is necessary when the dataset size is sufficiently large. We use the Sepsis-POMDP domain with 200, 1000, and 5000 patients. We show the best policies that are most frequently selected by our approach in Figure~\ref{fig:heatmap_benefit_split}(b). Unsurprisingly, policies trained on larger datasets perform better. In the 200-patient dataset, having \textbf{\ssrrrs 5-split} is crucial in picking the best policy, as most policies perform quite poorly. The gap between different approaches becomes smaller with 1000 patients, and even smaller when there are 5000 patients in the dataset. However, it is worth noting that even in the large dataset regime (N=5000), \textbf{\ssrrrs} still outperforms the One-Split OPE method in selecting the best algorithm.


\textbf{Additional Analysis.} Our method \ssrrrs can also be used to select hyperparameters for a single algorithm, as we demonstrate in Appendix~\ref{ap:robustness}. 
One might also wonder how sensitive is \ssrrrs pipeline to the choice of OPE method used inside the pipeline. OPE methods are known to significantly vary in accuracy for different domains, and unsurprisingly, using a reasonable OPE method for the domain is important (see Appendix~\ref{ap:ope-sensitivity}). Note that the OPE estimators we use in our results are very popular ones, and it is possible to use standard approaches, though additional benefits may come from using even better OPE methods. Finally, related to this question, one might wonder if particular OPE methods might be biased towards certain OPL algorithms which make similar assumptions (such as assuming a Markov structure): interestingly in preliminary experiments, FQE estimators did not seem to give FQI algorithms higher performance estimations (see Appendix~\ref{ap:fqe-fqi-bias}).

==> fvcxkgstnhxcyccfvtcknzrmdvqdfdgy_arXiv/theorem.tex <==
\section{Advantage of Repeated Sampling in Offline Setting}
We now demonstrate why it is important to conduct repeated sampling on the dataset and why it is particularly important for offline RL. Consider a finite set of $J$ offline RL algorithms $\mathcal{A}$. Let the policy produced by algorithm $\mathcal{A}_j$ on training dataset $\mathcal{D}$ be $\pi_j$, its estimated performance on a test set $\hat{V}^{\pi_j}$,  and its true (unknown) value be $V^{\pi_j}.$ Denote the true best resulting policy as $\pi_{j^*} = \argmax_j V^{\pi_j}$ and the corresponding algorithm $\mathcal{A}_{j^*}$. Let the best policy picked based on its test set performance as $\pi_{\hat{j}^*} = \argmax_j \hat{V}^{\pi_j}$ and the corresponding algorithm $\mathcal{A}_{\hat{j}^*}$. 
\begin{theorem}
\label{thm:benefit_n_splits} 
Then there exists stochastic decision processes and datasets such that (i) using a single train/test split procedure will select a suboptimal policy and algorithm with significant finite probability,  $P(\pi_{\hat{j}^*} \neq \pi_{j^*}) \geq C$, with corresponding substantial loss in performance $O(V_{max})$, and, in contrast,  (ii) averaging across $N_s$ train/test splits will select the optimal policy with probability 1: $\lim_{N_s\to\infty} P(\pi_{\hat{j}^*} = \pi_{j^*}) \to 1.$
\end{theorem}
\begin{proof}
We proceed by constructing a stochastic decision process. A common domain to illustrate the importance of strategic exploration is a chain MDP. Here consider an episodic, finite horizon, finite chain, deterministic decision process with 5 states, $s_1,\ldots,s_5$, with two actions. $a_1$ moves the state one down except for at the starting state, and $a_2$ increments the state one up except for the final state: more formally,  $p(s_{i-1}|s_i,a_1)=1$ except for $p(s_1|s_1,a_1)=1$; $p(s_{i+1}|s_i,a_2)$ except for $p(s_5|s_t,a_2)=1$. The reward is 0 in all states except $R(s_1)=0.2$ and $R(s_5)=101$. All episodes are length $H=5$  and start in state $s_1$. The optimal policy always takes $a_2$ and achieves $V_{max}=R(s_5).$ Any other policy achieves at most $H*0.2=1$ reward.  

The behavior policy is uniform random over the two actions, $\pi_b(a_1|s)=0.5=\pi_b(a_2).$ Let the available offline dataset $D$ consist of 200 episodes gathered using $\pi_b.$ Given the behavior policy, each of the 32$=2^5$ unique trajectories has an equal probability of being observed, and only one of these $\tau_h=(s_1,0,a_2,s_2,0,a_2,,s_3,0,a_2,s_4,0,a_2,s5,101)$ achieves the highest return. On average out of 200 episodes\footnote{Our calculations can easily be extended to cases where there are different numbers of observed $\tau_h$, but for simplicity we assume a dataset where the average expected number of $\tau_h$ are observed.}, 6 (=$round(200/32)$) episodes will match $\tau_h$. All other episodes will have a return of 1 or less. 

Let there be a set of $H$ offline RL algorithms $\mathcal{A}_h$, each which optimizes the reward over a different horizon $h=1:H$, by constructing a maximum-likelihood estimate (MLE) MDP model $\mathcal{M}$ given a training dataset $D_{tr}$, and then computing a policy $\pi_h$ that optimizes the $h$-step value given the learned MDP  $\mathcal{M}$ model\footnote{During planning with the learned MDP model, we restrict taking the maximum value over actions for a given state $s$ to only actions that have been taken at least once in that state in the dataset, e.g. $\max_{a \,s.t.\, n(s,a) \geq 1}$, where $n(s,a)$ is the counts of the number of times action $a$ was taken in state $s$ in the dataset. Note that in a finite dataset, some states and/or actions may not be observed, and this common choice simply ensures that the algorithm does not overestimate the value of untried actions.}
For example, algorithm $\mathcal{A}_2$ will take the MLE MDP model and construct a policy to optimize the sum over rewards for the next two time steps $\pi_2(s) = \arg\max_a r(s) + \sum_{s'} p(s'|s,a) r(s').$ We think this is a reasonable set of algorithms to consider as an illustrative example: the horizon length can directly influence the amount of data needed to compute an optimal policy, and recent work has explored using shorter horizons (**cite Cheng, Adith), so choosing the right horizon can be viewed as a bias/variance tradeoff, suitable for automatic model selection. 

Observe that even if given access to the true (unknown) MDP parameters, algorithms $\mathcal{A}_1,\ldots,\mathcal{A}_4$ will compute a policy that is suboptimal: due to the shortened horizon length, to optimize the expected total reward, the resulting policy computed for $s_1$ will be $\pi_h(s_1)=\pi_1(s_1)=a_1$ for these algorithms $\mathcal{A}_h$, $h=1:4$. As the MDP is deterministic, this will also be true for any input dataset. 


We now consider the impacts of partitioning the input dataset into a training dataset $D_{tr}$ taken as input by each algorithm $\mathcal{A}_h$ to compute a policy $\pi_{\hat{h}}$, and an evaluation/test dataset $D_{te}$: $D= D_{tr} \cup D_{te}$. For algorithm  $\mathcal{A}_5$ to learn the optimal policy $\pi^*$ which achieves $V_{max}$, it must learn over a dataset $D_{tr}$ that includes one or more examples of the highest return trajectory $\tau_h$. Note that a single episode of $\tau_h$ in the training set is sufficient to learn the optimal policy\footnote{A single example of $\tau_h$ will induce a MLE $\hat{\mathcal{M}}$ with the correct reward model for all states, and the dynamics model for action $a_2$. From the procedure used to compute an optimal policy $\hat{\mathcal{M}}$, this will result in an optimal policy.}.

Assume that the offline evaluation of the policies learned by the algorithm on $D_{tr}$ is performed using importance sampling on $D_{te}$: note, our results will still apply, with minor modifications, if off policy evaluation is performed on $D_{te}$ using fitted Q evaluation (**cite Cameron / Yisong) or using a certainty-equivalent MDP constructed from $D_{te}$. 

Then the off policy evaluation of the policy learned by the full horizon algorithm $\mathcal{A}_5$, $\hat{V}^{\pi_5}(s_1)$, will only be greater than 1 if there also exists at least one episode of the highest return trajectory $\tau_h$. 

Assume the training dataset and test dataset are constructed by randomly sampling 50\% of the episodes to be in each. By assumption, there are 6 samples of $\tau_h$, which have an equal chance of being in either the training or test set. There are 7=6+1 ways to partition the 6 exchangable episodes of $\tau_h$ into the training and test sets $([6,0],[5,1],[4,2],[3,3],[2,4], [1, 5],[0,6])$. 
Since the training and test set are identical in size (100 trajectories each), and we only care about whether a trajectory $\tau$ is identical to $\tau_h$ or not, each of those 7 partitions happens with equal probability.

From the above analysis, $\mathcal{A}_5$ can only learn an optimal policy, and its estimated value $\hat{V}^{\pi_5}> 1$ on $D_{te}$ if there is at least one $\tau_h$ in both the training and test set datasets, which occurs in partitions $([5,1],[4,2],[3,3], [2,4], [1,5])$. This occurs with probability $\frac{5}{7}$. Otherwise, either (a) $\mathcal{A}_5$ will not learn an optimal policy, and instead will learn $\pi_5(s_1) = \pi_1(s_1)=a_1$, or (b) $\mathcal{A}_5$ will learn an optimal policy $\pi_5(s_1)=a_2$ but as the test dataset does not contain  $\tau_h$, $\hat{V}^{\pi_5} = 0.2 < \hat{V}^{\pi_1}$. In both cases, the selected policy given its performance on the test set will be $\pi_1(s_1)=a_1$. The resulting loss in performance is $V_{max} - V^{\pi_1} = V_{\max} - 1 = O(V_{\max}).$ This failure occurs with substantial probability $\frac{2}{7}= 28.57\%$. This proves part (i) of the theorem. 

To prove part (ii) of the proof, we consider cases where at least one $\tau_h$ is in both $D_{tr}$ and $D_{te}$.  Note 
$\hat{V}^{\pi_1} \leq \frac{R(s_1)}{1/32} = \frac{1}{1/32}$.  Define $E_{ss}$ as a "successful split": the event that 2 or more of $\tau_h$ (high resturn) episodes are in $D_{te}$, but not all 6. On event $E_{ss}$,  the optimal policy (which will be computed by $\mathcal{A}_5$ on the training set), will have an estimated value on $D_{te}$, using importance sampling:
\begin{equation}
\hat{V}^{\pi^*}_{ss} \geq \frac{2}{|D_{te}|} \frac{R(s_5)}{1/32}  = \frac{2}{1/32}*\frac{101}{100} > 2 \hat{V}^{\pi_1} \label{eqn:vpi1}
\end{equation}
since there are at least $2$ $\tau_h$ trajectories, each with propensity weight $\frac{1}{1/32}$ and reward $R(s_5)$. 
Therefore on Event $E_{ss}$ the optimal policy can be learned and estimated as having high reward. The probability of event $E_{ss}$ is greater than 0.5: $P(E_{ss}) = \frac{4}{7}.$ 

In the repeated train-test split setting, the algorithm selected is the one that has the best performance on the test set, on average across all $N_s$ splits. Let $E_{h}$ be the event that at least half the train-test dataset splits are successful (Event $E_{ss}$ holds for that split). In this case then the average performance of $\mathcal{A}_5$ will be at least
\begin{eqnarray*}
\hat{V}_{\mathcal{A}_5} &\geq& \frac{1}{N_s} \left( \frac{N_s}{2} \hat{V}^{\pi^*}_{ss} + 0 \right) \\
&\geq& \frac{1}{N_s} \left( \frac{N_s}{2} 2 \hat{V}^{\pi_1} + 0 \right) \\
&=& \hat{V}^{\pi_1},
\end{eqnarray*}
where the first line uses a lower bound of 0 when the event $E_{ss}$ fails to hold, and substitutes in Equation~\ref{eqn:vpi1}. Therefore as long as event $E_h$ holds, the optimal policy $\pi^*$ (which will be computed by algorithm $\mathcal{A}_5$ will be selected. Since $P(E_{ss}) > 0.5$, the probability\footnote{Even for small values of $N_s$ this still holds with high probability. For this particular example, though if $N_s=1$, the failure probability is $28.57\%$, if $N_s = 10$, then the failure probability is only 12\%. (**EB-- check numbers again).} as the number of splits goes to infinity that $E_{ss}$ holds on least half of those splits goes to 1: $\lim_{N_s \to \infty} P (E_h) \to 1$. 











\end{proof}




==> fvcxkgstnhxcyccfvtcknzrmdvqdfdgy_arXiv/thm_and_proof.tex <==
Consider a finite set of $J$ offline RL algorithms $\mathcal{A}$. Let the policy produced by algorithm $\mathcal{A}_j$ on training dataset $\mathcal{D}$ be $\pi_j$, its estimated performance on a validation set $\hat{V}^{\pi_j}$,  and its true (unknown) value be $V^{\pi_j}.$ Denote the true best resulting policy as $\pi_{j^*} = \argmax_j V^{\pi_j}$ and the corresponding algorithm $\mathcal{A}_{j^*}$. Let the best policy picked based on its validation set performance as $\pi_{\hat{j}^*} = \argmax_j \hat{V}^{\pi_j}$ and the corresponding algorithm $\mathcal{A}_{\hat{j}^*}$.

\textbf{Theorem 1. }\textit{Then there exist stochastic decision processes and datasets such that (i) using a single train/validation split procedure will select a suboptimal policy and algorithm with significant finite probability, $P(\pi_{\hat{j}^*} \neq \pi_{j^*}) \geq C$, with corresponding substantial loss in performance $O(V_{max})$, and, in contrast,  (ii) averaging across $N_s$ train/validation splits will select the optimal policy with probability 1: $\lim_{N_s\to\infty} P(\pi_{\hat{j}^*} = \pi_{j^*}) \to 1.$}
\begin{proof}
We proceed by constructing a stochastic decision process. A common domain to illustrate the importance of strategic exploration is a chain MDP. Here consider an episodic, finite horizon, finite chain, deterministic decision process with 6 states, $s_1,\ldots,s_H$, ($H=6$) with two actions. $a_1$ moves the state one down except for at the starting state, and $a_2$ increments the state one up except for the final state: more formally,  $p(s_{i-1}|s_i,a_1)=1$ except for $p(s_1|s_1,a_1)=1$; $p(s_{i+1}|s_i,a_2)$ except for $p(s_H|s_H,a_2)=1$. The reward is 0 in all states except $R(s_1)=1/6$ and $R(s_H)=201$. All episodes are length $H=6$  and start in state $s_1$. The optimal policy always takes $a_2$ and achieves $V_{max}=R(s_H).$ Any other policy achieves at most $H*1/6=1$ reward.  

The behavior policy is uniform random over the two actions, $\pi_b(a_1|s)=0.5=\pi_b(a_2).$ Let the available offline dataset $D$ consist of 200 episodes gathered using $\pi_b.$ Given the behavior policy, each of the 64$=2^H$ unique trajectories has an equal probability of being observed, and only one of these $\tau_h=(s_1,0,a_2,s_2,0,a_2,,s_3,0,a_2,s_4,0,a_2,s_5,a_2,s_H,R(s_H))$ achieves the highest return. On average out of 200 episodes\footnote{Our calculations can easily be extended to cases where there are different numbers of observed $\tau_h$, but for simplicity we assume a dataset where the average expected number of $\tau_h$ are observed.}, $n_{\tau_h}$=3(=$round(|\mathcal{D}|/(2^H))$) episodes will match $\tau_h$. All other episodes will have a return of 1 or less.

Let there be a set of $H$ offline RL algorithms $\mathcal{A}_h$, each which optimizes the reward over a different horizon $h=1:H$, by constructing a maximum-likelihood estimate (MLE) MDP model $\mathcal{M}$ given a training dataset $D_{tr}$, and then computing a policy $\pi_h$ that optimizes the $h$-step value given the learned MDP  $\mathcal{M}$ model\footnote{During planning with the learned MDP model, we restrict taking the maximum value over actions for a given state $s$ to only actions that have been taken at least once in that state in the dataset, e.g. $\max_{a \,s.t.\, n(s,a) \geq 1}$, where $n(s,a)$ is the counts of the number of times action $a$ was taken in state $s$ in the dataset. Note that in a finite dataset, some states and/or actions may not be observed, and this common choice simply ensures that the algorithm does not overestimate the value of untried actions.}
For example, algorithm $\mathcal{A}_2$ will take the MLE MDP model and construct a policy to optimize the sum over rewards for the next two time steps $\pi_2(s) = \arg\max_a r(s) + \sum_{s'} p(s'|s,a) r(s').$ We think this is a reasonable set of algorithms to consider as an illustrative example: the horizon length can directly influence the amount of data needed to compute an optimal policy, and recent work has explored using shorter horizons~\citep{cheng2021heuristic,mazoure2021improving,liao2020personalized}, so choosing the right horizon can be viewed as a bias/variance tradeoff, suitable for automatic model selection. 

Observe that even if given access to the true (unknown) MDP parameters, algorithms $\mathcal{A}_1,\ldots,\mathcal{A}_{H-1}$ will compute a policy that is suboptimal: due to the shortened horizon length, to optimize the expected total reward, the resulting policy computed for $s_1$ will be $\pi_h(s_1)=\pi_1(s_1)=a_1$ for these algorithms $\mathcal{A}_h$, $h=1:{H-1}$. As the MDP is deterministic, this will also be true for any input dataset. 


We now consider the impacts of partitioning the input dataset into a training dataset $D_{tr}$ taken as input by each algorithm $\mathcal{A}_h$ to compute a policy $\pi_{\hat{h}}$, and an evaluation/test dataset $D_{te}$: $D= D_{tr} \cup D_{te}$. For algorithm  $\mathcal{A}_H$ to learn the optimal policy $\pi^*$ which achieves $V_{max}$, it must learn over a dataset $D_{tr}$ that includes one or more examples of the highest return trajectory $\tau_h$. Note that a single episode of $\tau_h$ in the training set is sufficient to learn the optimal policy\footnote{A single example of $\tau_h$ will induce a MLE $\hat{\mathcal{M}}$ with the correct reward model for all states, and the dynamics model for action $a_2$. From the procedure used to compute an optimal policy $\hat{\mathcal{M}}$, this will result in an optimal policy.}.

Assume that the offline evaluation of the policies learned by the algorithm on $D_{tr}$ is performed using importance sampling on $D_{te}$: note, our results will still apply, with minor modifications, if off policy evaluation is performed on $D_{te}$ using fitted Q evaluation~\citep{le2019batch} or using a certainty-equivalent MDP constructed from $D_{te}$. 

Then the off policy evaluation of the policy learned by the full horizon algorithm $\mathcal{A}_H$, $\hat{V}^{\pi_H}(s_1)$, will only be greater than 1 if there also exists at least one episode of the highest return trajectory $\tau_h$. 

Assume the training dataset and validation dataset are constructed by randomly sampling 50\% of the episodes to be in each. By assumption, there are $n_{\tau_h}$ samples of $\tau_h$, which have an equal chance of being in either the training or validation set. There are $n_{\tau_h}+1$ ways to partition the $n_{\tau_h}$ exchangable episodes of $\tau_h$ into the training and validation sets, here $([3,0],[2,1],[1,2],[0,3])$. Note the training and validation set are identical in size ($|\mathcal{D}|/2$ trajectories each), and we only care about whether a trajectory $\tau$ is identical to $\tau_h$ or not. The probability that each of these partitions occurs is : $P([3,0]) = P([0,3]) = \frac{100}{200}*\frac{99}{199}*\frac{98}{198}\approx 0.123$. 



From the above analysis, $\mathcal{A}_H$ can only learn an optimal policy, and its estimated value $\hat{V}^{\pi_5}> 1$ on $D_{te}$ if there is at least one $\tau_h$ in both the training and validation set datasets, which occurs in partitions $([2,1],[1,2])$. This occurs with probability $0.754$. Otherwise, either (a) $\mathcal{A}_H$ will not learn an optimal policy, and instead will learn $\pi_H(s_1) = \pi_1(s_1)=a_1$, or (b) $\mathcal{A}_H$ will learn an optimal policy $\pi_H(s_1)=a_2$ but as the validation dataset does not contain  $\tau_h$, $\hat{V}^{\pi_H} = 1/H < \hat{V}^{\pi_1}$. In both cases, the selected policy given its performance on the validation set will be $\pi_1(s_1)=a_1$. The resulting loss in performance is $V_{max} - V^{\pi_1} = V_{\max} - 1 = O(V_{\max}).$ This failure occurs with substantial probability $24.6\%$. This proves part (i) of the theorem. 

To prove part (ii) of the proof, we consider cases where at least one $\tau_h$ is in both $D_{tr}$ and $D_{te}$.  Note 
$\hat{V}^{\pi_1} \leq \frac{R(s_1)}{1/2^H} = \frac{1}{1/2^H}$.  Define $E_{ss}$ as a "successful split": the event that 1 or more of $\tau_h$ (high returns) episodes are in $D_{te}$, but not all $n_{\tau_h}$. On event $E_{ss}$,  the optimal policy (which will be computed by $\mathcal{A}_H$ on the training set), will have an estimated value on $D_{te}$, using importance sampling:
\begin{equation}
\hat{V}^{\pi^*}_{ss} \geq \frac{1}{|D_{te}|} \frac{R(s_H)}{1/2^H}  = \frac{1}{1/2^H}*\frac{201}{100} > 2 \hat{V}^{\pi_1} \label{eqn:vpi1}
\end{equation}
since there are at least $1$ $\tau_h$ trajectories, each with propensity weight $\frac{1}{1/2^H}$ and reward $R(s_H)$. 
Therefore on Event $E_{ss}$ the optimal policy can be learned and estimated as having high reward. The probability of event $E_{ss}$ is greater than 0.5: $P(E_{ss}) = 0.754.$ 

In the repeated train-validation split setting, the algorithm selected is the one that has the best performance on the validation set, on average across all $N_s$ splits. Let $E_{h}$ be the event that at least half the train-validation dataset splits are successful (Event $E_{ss}$ holds for that split). In this case then the average performance of $\mathcal{A}_5$ will be at least
\begin{eqnarray*}
\hat{V}_{\mathcal{A}_5} &\geq& \frac{1}{N_s} \left( \frac{N_s}{2} \hat{V}^{\pi^*}_{ss} + 0 \right) \\
&\geq& \frac{1}{N_s} \left( \frac{N_s}{2} 2 \hat{V}^{\pi_1} + 0 \right) \\
&=& \hat{V}^{\pi_1},
\end{eqnarray*}
where the first line uses a lower bound of 0 when the event $E_{ss}$ fails to hold, and substitutes in Equation~\ref{eqn:vpi1}. Therefore as long as event $E_h$ holds, the optimal policy $\pi^*$ (which will be computed by algorithm $\mathcal{A}_H$ will be selected. Since $P(E_{ss}) > 0.5$, the probability\footnote{**calculate for finite S.} as the number of splits goes to infinity that $E_{ss}$ holds on least half of those splits goes to 1: $\lim_{N_s \to \infty} P (E_h) \to 1$. 










\vfill
\end{proof}




==> pseudocode.tex <==
\begin{algorithm}[t]
\SetAlgoLined
\SetKwFunction{subsample}{Subsample}
\SetKwFunction{append}{append}
% \SetKwInOut{Parameter}{Parameters: }
\KwIn{offline RL data $\data$; A set of AH pairs [$\gA_1, \gA_2, ..., \gA_z$], an OPE estimator  $\widehat V$, and choose a split number $K\in \mathbb{N}$.}
%\Parameter{hidden labels $\mathbf{y}^u$, $\bm{\theta} = (\bm{\theta}_Y, \bm{\theta}_E)$}
\KwOut{policy $\hat \pi^*$ for deployment}
\BlankLine
% $t \leftarrow 0$\\
% $\hat{\bm{\theta}}_Y^{(0)}\leftarrow \argmin \text{NLL}(\bm{\theta}_Y|\mathbf{y}^l)$\\
% $\hat{\bm{\theta}}_E^{(0)}\leftarrow \argmin \text{NLL}(\bm{\theta}_E|\mathbf{y}^l)$\\
$\gR$ = []  \Comment{\textcolor{red}{The split step}}\\
\For{$i \leftarrow 1...K$}{
    $R^\mathrm{train}_i, R^\mathrm{valid}_i = $ \subsample($\data, 0.5$)
    $\gR = \gR \cup (R^\mathrm{train}_i, R^\mathrm{valid}_i)$
}
$\gG$ = []  \Comment{\textcolor{red}{The select step}}\\
\For{$i \leftarrow 1...z$}{
    $\gS$ = [] \\
    \For{$j \leftarrow 1...K$}{
        $\pi_i = \mathcal{A}(R^\mathrm{train}_j)$ \\
        $\theta_j = \widehat V(\pi_i; R^\mathrm{valid}_j)$ \\
        $\gS = \gS \cup \theta_j$ \\
    %   $\mathbf{y}^{(t)} \leftarrow \mathbb{I}\{p(\mathbf{y}|\mathbf{X}^u_C, \mathbf{X}^u_E; \bm{\theta}_Y^{(t)}, \bm{\theta}_E^{(t)}) > 0.5\}$\\
    %   $\hat{\bm{\theta}}_Y^{(t+1)}\leftarrow \argmin \text{NLL}(\bm{\theta}_Y|\mathbf{y}^l,\mathbf{y}^{(t)})$\\
    %   $\hat{\bm{\theta}}_E^{(t+1)}\leftarrow \argmin \text{NLL}(\bm{\theta}_E|\mathbf{y}^l,\mathbf{y}^{(t)})$\\
    %     $t \leftarrow t+1$\\
     }
     $\gG = \gG \cup \frac{1}{K} \sum_{j=1}^K \gS_j$ \Comment{\small{\textcolor{red}{One score per algorithm}}}
 }
  $\gA^* = \gA_{o+}$ where $o = \argmax(\gG)$ \Comment{\small{\textcolor{red}{Choose the highest}}}\\
%  $\gA^* = [\gA_1, \gA_2, ..., \gA_z]_{\argmax(\gG)}$ \Comment{\small{\textcolor{red}{Choose highest}}} \\
 $\pi^* = \gA^*(\data)$ \Comment{\textcolor{red}{The full retrain step}} \\
 \Return{$\pi^*$}
 \caption{Split-Select-Retrain with Repeated Random Sub-sampling (SSR-RS)}
 \label{alg:ssr-rs}
\end{algorithm}

==> theorem.tex <==
\section{Advantage of Repeated Sampling in Offline Setting}
% this is jonathan's suggestion
We now demonstrate why it is important to conduct repeated sampling on the dataset and why it is particularly important for offline RL. Consider a finite set of $J$ offline RL algorithms $\mathcal{A}$. Let the policy produced by algorithm $\mathcal{A}_j$ on training dataset $\mathcal{D}$ be $\pi_j$, its estimated performance on a test set $\hat{V}^{\pi_j}$,  and its true (unknown) value be $V^{\pi_j}.$ Denote the true best resulting policy as $\pi_{j^*} = \argmax_j V^{\pi_j}$ and the corresponding algorithm $\mathcal{A}_{j^*}$. Let the best policy picked based on its test set performance as $\pi_{\hat{j}^*} = \argmax_j \hat{V}^{\pi_j}$ and the corresponding algorithm $\mathcal{A}_{\hat{j}^*}$. 
\begin{theorem}
\label{thm:benefit_n_splits} 
Then there exists stochastic decision processes and datasets such that (i) using a single train/test split procedure will select a suboptimal policy and algorithm with significant finite probability,  $P(\pi_{\hat{j}^*} \neq \pi_{j^*}) \geq C$, with corresponding substantial loss in performance $O(V_{max})$, and, in contrast,  (ii) averaging across $N_s$ train/test splits will select the optimal policy with probability 1: $\lim_{N_s\to\infty} P(\pi_{\hat{j}^*} = \pi_{j^*}) \to 1.$
\end{theorem}
% by proof by example, 
\begin{proof}
We proceed by constructing a stochastic decision process. A common domain to illustrate the importance of strategic exploration is a chain MDP. Here consider an episodic, finite horizon, finite chain, deterministic decision process with 5 states, $s_1,\ldots,s_5$, with two actions. $a_1$ moves the state one down except for at the starting state, and $a_2$ increments the state one up except for the final state: more formally,  $p(s_{i-1}|s_i,a_1)=1$ except for $p(s_1|s_1,a_1)=1$; $p(s_{i+1}|s_i,a_2)$ except for $p(s_5|s_t,a_2)=1$. The reward is 0 in all states except $R(s_1)=0.2$ and $R(s_5)=101$. All episodes are length $H=5$  and start in state $s_1$. The optimal policy always takes $a_2$ and achieves $V_{max}=R(s_5).$ Any other policy achieves at most $H*0.2=1$ reward.  

The behavior policy is uniform random over the two actions, $\pi_b(a_1|s)=0.5=\pi_b(a_2).$ Let the available offline dataset $D$ consist of 200 episodes gathered using $\pi_b.$ Given the behavior policy, each of the 32$=2^5$ unique trajectories has an equal probability of being observed, and only one of these $\tau_h=(s_1,0,a_2,s_2,0,a_2,,s_3,0,a_2,s_4,0,a_2,s5,101)$ achieves the highest return. On average out of 200 episodes\footnote{Our calculations can easily be extended to cases where there are different numbers of observed $\tau_h$, but for simplicity we assume a dataset where the average expected number of $\tau_h$ are observed.}, 6 (=$round(200/32)$) episodes will match $\tau_h$. All other episodes will have a return of 1 or less. 

Let there be a set of $H$ offline RL algorithms $\mathcal{A}_h$, each which optimizes the reward over a different horizon $h=1:H$, by constructing a maximum-likelihood estimate (MLE) MDP model $\mathcal{M}$ given a training dataset $D_{tr}$, and then computing a policy $\pi_h$ that optimizes the $h$-step value given the learned MDP  $\mathcal{M}$ model\footnote{During planning with the learned MDP model, we restrict taking the maximum value over actions for a given state $s$ to only actions that have been taken at least once in that state in the dataset, e.g. $\max_{a \,s.t.\, n(s,a) \geq 1}$, where $n(s,a)$ is the counts of the number of times action $a$ was taken in state $s$ in the dataset. Note that in a finite dataset, some states and/or actions may not be observed, and this common choice simply ensures that the algorithm does not overestimate the value of untried actions.}
For example, algorithm $\mathcal{A}_2$ will take the MLE MDP model and construct a policy to optimize the sum over rewards for the next two time steps $\pi_2(s) = \arg\max_a r(s) + \sum_{s'} p(s'|s,a) r(s').$ We think this is a reasonable set of algorithms to consider as an illustrative example: the horizon length can directly influence the amount of data needed to compute an optimal policy, and recent work has explored using shorter horizons (**cite Cheng, Adith), so choosing the right horizon can be viewed as a bias/variance tradeoff, suitable for automatic model selection. 

Observe that even if given access to the true (unknown) MDP parameters, algorithms $\mathcal{A}_1,\ldots,\mathcal{A}_4$ will compute a policy that is suboptimal: due to the shortened horizon length, to optimize the expected total reward, the resulting policy computed for $s_1$ will be $\pi_h(s_1)=\pi_1(s_1)=a_1$ for these algorithms $\mathcal{A}_h$, $h=1:4$. As the MDP is deterministic, this will also be true for any input dataset. 

%This policy has corresponding  $V^{\pi_h}=1$.

We now consider the impacts of partitioning the input dataset into a training dataset $D_{tr}$ taken as input by each algorithm $\mathcal{A}_h$ to compute a policy $\pi_{\hat{h}}$, and an evaluation/test dataset $D_{te}$: $D= D_{tr} \cup D_{te}$. For algorithm  $\mathcal{A}_5$ to learn the optimal policy $\pi^*$ which achieves $V_{max}$, it must learn over a dataset $D_{tr}$ that includes one or more examples of the highest return trajectory $\tau_h$. Note that a single episode of $\tau_h$ in the training set is sufficient to learn the optimal policy\footnote{A single example of $\tau_h$ will induce a MLE $\hat{\mathcal{M}}$ with the correct reward model for all states, and the dynamics model for action $a_2$. From the procedure used to compute an optimal policy $\hat{\mathcal{M}}$, this will result in an optimal policy.}.

Assume that the offline evaluation of the policies learned by the algorithm on $D_{tr}$ is performed using importance sampling on $D_{te}$: note, our results will still apply, with minor modifications, if off policy evaluation is performed on $D_{te}$ using fitted Q evaluation (**cite Cameron / Yisong) or using a certainty-equivalent MDP constructed from $D_{te}$. 

Then the off policy evaluation of the policy learned by the full horizon algorithm $\mathcal{A}_5$, $\hat{V}^{\pi_5}(s_1)$, will only be greater than 1 if there also exists at least one episode of the highest return trajectory $\tau_h$. 

Assume the training dataset and test dataset are constructed by randomly sampling 50\% of the episodes to be in each. By assumption, there are 6 samples of $\tau_h$, which have an equal chance of being in either the training or test set. There are 7=6+1 ways to partition the 6 exchangable episodes of $\tau_h$ into the training and test sets $([6,0],[5,1],[4,2],[3,3],[2,4], [1, 5],[0,6])$. 
Since the training and test set are identical in size (100 trajectories each), and we only care about whether a trajectory $\tau$ is identical to $\tau_h$ or not, each of those 7 partitions happens with equal probability.

From the above analysis, $\mathcal{A}_5$ can only learn an optimal policy, and its estimated value $\hat{V}^{\pi_5}> 1$ on $D_{te}$ if there is at least one $\tau_h$ in both the training and test set datasets, which occurs in partitions $([5,1],[4,2],[3,3], [2,4], [1,5])$. This occurs with probability $\frac{5}{7}$. Otherwise, either (a) $\mathcal{A}_5$ will not learn an optimal policy, and instead will learn $\pi_5(s_1) = \pi_1(s_1)=a_1$, or (b) $\mathcal{A}_5$ will learn an optimal policy $\pi_5(s_1)=a_2$ but as the test dataset does not contain  $\tau_h$, $\hat{V}^{\pi_5} = 0.2 < \hat{V}^{\pi_1}$. In both cases, the selected policy given its performance on the test set will be $\pi_1(s_1)=a_1$. The resulting loss in performance is $V_{max} - V^{\pi_1} = V_{\max} - 1 = O(V_{\max}).$ This failure occurs with substantial probability $\frac{2}{7}= 28.57\%$. This proves part (i) of the theorem. 

To prove part (ii) of the proof, we consider cases where at least one $\tau_h$ is in both $D_{tr}$ and $D_{te}$.  Note 
$\hat{V}^{\pi_1} \leq \frac{R(s_1)}{1/32} = \frac{1}{1/32}$.  Define $E_{ss}$ as a "successful split": the event that 2 or more of $\tau_h$ (high resturn) episodes are in $D_{te}$, but not all 6. On event $E_{ss}$,  the optimal policy (which will be computed by $\mathcal{A}_5$ on the training set), will have an estimated value on $D_{te}$, using importance sampling:
\begin{equation}
\hat{V}^{\pi^*}_{ss} \geq \frac{2}{|D_{te}|} \frac{R(s_5)}{1/32}  = \frac{2}{1/32}*\frac{101}{100} > 2 \hat{V}^{\pi_1} \label{eqn:vpi1}
\end{equation}
since there are at least $2$ $\tau_h$ trajectories, each with propensity weight $\frac{1}{1/32}$ and reward $R(s_5)$. 
Therefore on Event $E_{ss}$ the optimal policy can be learned and estimated as having high reward. The probability of event $E_{ss}$ is greater than 0.5: $P(E_{ss}) = \frac{4}{7}.$ 

In the repeated train-test split setting, the algorithm selected is the one that has the best performance on the test set, on average across all $N_s$ splits. Let $E_{h}$ be the event that at least half the train-test dataset splits are successful (Event $E_{ss}$ holds for that split). In this case then the average performance of $\mathcal{A}_5$ will be at least
\begin{eqnarray*}
\hat{V}_{\mathcal{A}_5} &\geq& \frac{1}{N_s} \left( \frac{N_s}{2} \hat{V}^{\pi^*}_{ss} + 0 \right) \\
&\geq& \frac{1}{N_s} \left( \frac{N_s}{2} 2 \hat{V}^{\pi_1} + 0 \right) \\
&=& \hat{V}^{\pi_1},
\end{eqnarray*}
where the first line uses a lower bound of 0 when the event $E_{ss}$ fails to hold, and substitutes in Equation~\ref{eqn:vpi1}. Therefore as long as event $E_h$ holds, the optimal policy $\pi^*$ (which will be computed by algorithm $\mathcal{A}_5$ will be selected. Since $P(E_{ss}) > 0.5$, the probability\footnote{Even for small values of $N_s$ this still holds with high probability. For this particular example, though if $N_s=1$, the failure probability is $28.57\%$, if $N_s = 10$, then the failure probability is only 12\%. (**EB-- check numbers again).} as the number of splits goes to infinity that $E_{ss}$ holds on least half of those splits goes to 1: $\lim_{N_s \to \infty} P (E_h) \to 1$. 



%$\hat{V}^{\pi^*} \geq \hat{V}^{\[i_1}$

% put D in mathcal?
% check probabilities for partitioning
%
% need algorithm 5 to fail vs 1. 

% **EB:  the propensity weights are a bit clunky here. Maybe more all to MDP evaluation? But it's useful to show this works with IS too? 
%\frac{|D_{te}|}{|D_{te}|} \frac{H*R(s_1)}{1/32}  


% can our same example apply if use FQI or use a simulated MDP

% would this be easier to describe if use a MDP for offline evaluation? wouldn't have to worry about the dataset size

% 201 seems odd. can discuss later or move to FQI?


\end{proof}

% if truly Markov could have used a MDP to solve? 
% could one do this for a smaller gap? 

% show still true if use a different mechanism for picking, like including a lower bound 
% show a bound on the gap in performance? 

